Fast Fourier Intrinsic Network

We address the problem of decomposing an image into albedo and shading. We propose the Fast Fourier Intrinsic Network, FFI-Net in short, that operates in the spectral domain, splitting the input into several spectral bands. Weights in FFI-Net are optimized in the spectral domain, allowing faster convergence to a lower error. FFI-Net is lightweight and does not need auxiliary networks for training. The network is trained end-to-end with a novel spectral loss which measures the global distance between the network prediction and corresponding ground truth. FFI-Net achieves state-of-the-art performance on MPI-Sintel, MIT Intrinsic, and IIW datasets.

==> Makefile <==
# original Makefile by Pasi "okun" Valminen, 2004
# edited by Pekka "PQ" Paalanen, 2004 - 2007
# version 4.1.2007

## Modify these to your needs.

SHELL=/bin/bash

# document target basename
TARGET   := cvpr2018

# Autogenerated source files, like eps-figures created with
# gnuplot scripts. Target 'distclean' will delete files listed here.
AUTOTGT  := 
            

## The following should be ok as is.

# document source files
SRC      := $(wildcard *.tex) $(wildcard *.bib) $(AUTOTGT)

# programs
GS       := gs
TEXI2PDF := texi2pdf
GNUPLOT  := gnuplot
EPS2PDF  := epstopdf

GSPDF_OPTS := -sDEVICE=pdfwrite -dPDFSETTINGS=/printer \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true \
              -dEmbedAllFonts=true

# The GS options are from http://www.ctan.org/tex-archive/macros/latex/
#   contrib/IEEEtran/testflow/testflow_doc.txt

# Texi2pdf runs bibtex automatically and pdflatex as many times as needed.

all: $(TARGET).pdf

clean:
	rm -f *.{aux,bbl,blg,tmp,dvi,toc,log,out,idx,ilg,ind,brf,spl} *~

distclean: clean
	rm -f $(AUTOTGT) $(AUTOTGT:.pdf=.eps) $(TARGET).pdf

view: $(TARGET).pdf
	xpdf -remote view-$(abspath $(TARGET).pdf) $(TARGET).pdf &

%.pdf: %.tex $(SRC)
	$(TEXI2PDF) $<

%.eps: %.gp
	$(GNUPLOT) $<

%.pdf: %.eps
	epspdf $<
#	$(EPS2PDF) --nogs $< | $(GS) -q $(GSPDF_OPTS) \
#	  -dAutoRotatePages=/None -sOutputFile=$@ - -c quit

.SUFFIXES:
.PRECIOUS: %.dvi %.pdf
.DELETE_ON_ERROR: %.dvi %.pdf
.PHONY: all clean distclean view


==> WACV2021_ Fourier-Camera Ready/Makefile <==
# original Makefile by Pasi "okun" Valminen, 2004
# edited by Pekka "PQ" Paalanen, 2004 - 2007
# version 4.1.2007

## Modify these to your needs.

SHELL=/bin/bash

# document target basename
TARGET   := cvpr2018

# Autogenerated source files, like eps-figures created with
# gnuplot scripts. Target 'distclean' will delete files listed here.
AUTOTGT  := 
            

## The following should be ok as is.

# document source files
SRC      := $(wildcard *.tex) $(wildcard *.bib) $(AUTOTGT)

# programs
GS       := gs
TEXI2PDF := texi2pdf
GNUPLOT  := gnuplot
EPS2PDF  := epstopdf

GSPDF_OPTS := -sDEVICE=pdfwrite -dPDFSETTINGS=/printer \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true \
              -dEmbedAllFonts=true

# The GS options are from http://www.ctan.org/tex-archive/macros/latex/
#   contrib/IEEEtran/testflow/testflow_doc.txt

# Texi2pdf runs bibtex automatically and pdflatex as many times as needed.

all: $(TARGET).pdf

clean:
	rm -f *.{aux,bbl,blg,tmp,dvi,toc,log,out,idx,ilg,ind,brf,spl} *~

distclean: clean
	rm -f $(AUTOTGT) $(AUTOTGT:.pdf=.eps) $(TARGET).pdf

view: $(TARGET).pdf
	xpdf -remote view-$(abspath $(TARGET).pdf) $(TARGET).pdf &

%.pdf: %.tex $(SRC)
	$(TEXI2PDF) $<

%.eps: %.gp
	$(GNUPLOT) $<

%.pdf: %.eps
	epspdf $<
#	$(EPS2PDF) --nogs $< | $(GS) -q $(GSPDF_OPTS) \
#	  -dAutoRotatePages=/None -sOutputFile=$@ - -c quit

.SUFFIXES:
.PRECIOUS: %.dvi %.pdf
.DELETE_ON_ERROR: %.dvi %.pdf
.PHONY: all clean distclean view


==> WACV2021_ Fourier-Camera Ready/abstract.tex <==

\begin{abstract}
%This work addresses the problem of intrinsic image decomposition.We propose a Fast Fourier Intrinsic Network (FFI-Net) that operates in the spectral domain and introduces two important designs: 1) spectral banding for multi-scale processing from coarse (low frequency) to fine (high frequency) details, and 2) network weight optimization in the spectral domain (spectral residual blocks). FFI-Net achieves state-of-the-art performance on the benchmarks with dense ground truth, MPI-Sintel and MIT Intrinsic, and competitive results on the IIW dataset that contains only sparse ground truth (spectral banding not used).
We address the problem of decomposing an image into albedo and shading.
We propose the Fast Fourier Intrinsic Network,  FFI-Net in short, that
operates in the spectral domain, splitting the input into several spectral bands.
Weights in FFI-Net are optimized in the spectral domain, allowing faster
convergence to a lower error. FFI-Net is lightweight and does not need auxiliary networks for training.
The network is trained end-to-end with a novel spectral loss which measures the global distance between the network prediction and corresponding ground truth.
FFI-Net achieves state-of-the-art performance on MPI-Sintel, MIT Intrinsic, and IIW datasets.
\end{abstract}

==> WACV2021_ Fourier-Camera Ready/conclusion.tex <==
\section{Conclusion}
We proposed a Fast Fourier Intrinsic Network architecture (FFI-Net)
for intrinsic image decomposition. FFI-Net differs from the existing
works in the sense that inference and network training is
performed in the spectral domain and multi-scale learning is
implemented by spectral banding. The spectral residual blocks
introduced in this work converge faster and provide better accuracy than the conventional residual blocks. FFI-Net is lightweight and does not
need auxiliary networks for training. Our experiments with
three popular datasets verify that FFI-Net achieves state-of-the-art accuracy without auxiliary data training or
specific parameter tuning.
In the future work, we will explore the potential of spectral
network components in other image-to-image translation tasks such as depth estimation and spatial illumination estimation.

\medskip 

\para{Acknowledgement: } This work was partially supported by the National Natural Science
Foundation of China (NSFC) under Grant No. 61828602. 


==> WACV2021_ Fourier-Camera Ready/experiments.tex <==
\section{Experiments}\label{sec:expresults}

\para{Datasets.}
We conduct experiments on three popular datasets: {\em MPI-Sintel~\cite{butler2012naturalistic}}, {\em MIT Intrinsic~\cite{grosse2009ground}} and {\em IIW}~\cite{bell2014intrinsic}.
MPI-Sintel~\cite{butler2012naturalistic} consists of $18$ animated video clips of multiple scenes, each containing $40$ or $50$ frames. We experiment
with two different data splits:
\textit{image split}~\cite{narihira2015direct,fan2018revisiting,cheng2018intrinsic} and
\textit{scene split}~\cite{narihira2015direct,cheng2018intrinsic}.
% Following the previous work~\cite{narihira2015direct,lettry2018darn, cheng2018intrinsic}, the \textit{ResynthSintel} was used to satisfy $\mathcal I= \mathcal A \cdot \mathcal S$.
 MIT-Intrinsic~\cite{grosse2009ground} contains $20$ real objects in
$11$ different lighting configurations. The train/test split follows~\cite{barron2015shape}. IIW~\cite{bell2014intrinsic} has $5,230$ real images of mostly indoor scenes. Pairwise relative reflectance judgments are provided by humans as the ground truth albedo; the train/test split follows~\cite{fan2018revisiting}.  
%All split files are described in the supplementary material.

\vspace{\medskipamount}


%\vspace{-3mm}
\para{Training Details.}
For all datasets, we fix the number of spectral bands to
$M\!=\!5$ and use $N\!=\!10$ spectral residual blocks
for each band. \miaojing{Spectral residual blocks have the same configuration as the ordinary residual block~\cite{he2015deep} in terms of filter size, batch normalization, relu \etc. Training is conducted using the Adam optimizer with network weights randomly initialized.}
%Each spectral residual block chain is split into two branches after the $5$-th block to regress both the albedo and shading. %The convolutional layers in the residual blocks consist of $32$ $3\times3$ filters.
\textrm{(i)} For MPI Sintel, we randomly crop $384\times 384$ patch from each image. 
% To augment the training set, the cropped patches are flipped horizontally with $50\%$ probability and rotated randomly within $[-15, +15]$ degrees. 
The upper and lower bounds (Eq.\ref{eq:spectralbanding}) for each spectral band are $(384/4,384/2)$, $(384/8,384/4)$, $(384/16,384/8)$, $(384/32,384/16)$ and $(0,384/32)$, where $N_l = M_l$ and $N_u = M_u$ for square crops. We set the batch size to $4$ and the learning rate to \textrm{4e-4}. % multiplied by $0.5$ every $60$ epochs until $180$ epochs. 
\textrm{(ii)} For MIT Intrinsic with smaller images, we randomly crop $192\times192$ patches and flip them. The upper and lower bounds for each band are $(192/4,192/2)$, $(192/8,192/4)$, $(192/16,192/8)$, $(192/32,192/16)$ and $(0,192/32)$, respectively. The batch size is $8$ and learning rate is \textrm{8e-3}. %multiplied by $0.1$ every $100$ epochs until $200$ epochs. 
%For these two datasets, we use the unique network architecture but different learning rate and epoch numbers (detailed in supplement).
\textrm{(iii)} For IIW, we resize each image to $300\times 300$ as in~\cite{fan2018revisiting}; the batch size is set to $1$ and the learning rate is \textrm{1e-2}.
% with $90$ epochs. 
All networks are trained till convergences in our experiments.  

% \paragraph{Training Details} 
% \textrm{(i)} For MPI-Sintel, we randomly crop $384\times 384$ patches from each image. To augment the training set, the cropped patches are flipped horizontally with $50\%$ probability and rotated randomly within $[-15, +15]$ degrees. 
% We set the batch size to $4$; the initial learning rate
% is \textrm{4e-4} and is multiplied by $0.5$ every $60$ epochs until $180$ epochs. \textrm{(ii)} For MIT Intrinsic, images are in general smaller, we instead randomly crop $192\times192$ patches from each image and also flip. We set the batch size as $8$; the initial learning rate is \textrm{8e-4}, multiplied by $0.1$ every $100$ epochs until $200$ epochs. The same Adam optimizer is utilized in both datasets.  

\vspace{\medskipamount}

% \vspace{-3mm}
\para{Evaluation Protocol.} 
 We report results using the four common metrics: \textrm{(i)} \textit{si-MSE}: scale-invariant mean squared error (MSE);  \textrm{(ii)} \textit{si-LMSE}: scale-invariant local MSE, which uses sliding windows in si-MSE; the window size $w$ is usually 10\% of the larger dimension of the image while the sliding step is $0.5w$; \textrm{(iii)} \textit{DSSIM}: dissimilarity structural similarity index measure; it is made to correlate with the subjective image quality assessments~\cite{wang2004image}. For MIT, we also report the MSE and LMSE numbers which can be seen as variants of si-MSE and si-LMSE~\cite{grosse2009ground}. For IIW with sparse ground truth, we report the weighted human disagreement rate (WHDR)~\cite{bell2014intrinsic,fan2018revisiting}. 
 
 We compare our method with a number of prior arts; these approaches are trained in various ways including fully-/weakly-supervised learning~\cite{fan2018revisiting,cheng2018intrinsic,cgintrinsic,lettry2018darn,ma2018single,zhou2019glosh}, unsupervised learning~\cite{liu2020cvpr,grosse09intrinsic,bell2014intrinsic,bi20151}, as well as learning from auxiliary datasets~\cite{narihira2015direct,shi2017learning,cgintrinsic,zhou2019glosh} (see Sec.~\ref{sec:relatedwork}). We do not elaborate every detail with every method but mainly focus our comparison with those representative fully-supervised methods, \eg ~\cite{fan2018revisiting,cheng2018intrinsic,cgintrinsic,lettry2018darn}.  
%\textrm{(iv)} \textit{LMSE} (only for MIT Dataset); it is a variant of si-LMSE computed on albedo and shading to form a single metric~\cite{grosse2009ground}. 
%We use the Matlab evaluation kit provided by Fan \texit{et al.}~\cite{fan2018revisiting} for all evaluations.




\input{tab_mpi_scenesplit.tex}
\input{fig-mpi-scenesplit.tex}


\subsection{Results on MPI-Sintel}
Results for FFI-Net and various competing works
are shown in Tab.~\ref{tab:sintel_scene_split} (scene-split) and Tab.~\ref{tab:sintel_image_split} (image-split). 

The scene-split setting is more challenging as it requires generalization over unseen scenes. Tab.~\ref{tab:sintel_scene_split} shows that FFI-Net performs the best on most metrics. In particular, it achieves the best
average si-MSE, si-LMSE, and DSSIM of albedo and shading: 1.18, 0.73, and 8.77, respectively.  

FFI-Net achieves the best performance also for the image-split setting reported in Tab.~\ref{tab:sintel_image_split}, but with smaller margin.
We suggest a possible reason as the overfitting of deep networks on the 
shared contents between training and test images in image-split. This is illustrated
by the recent results in~\cite{kim2016unified,fan2018revisiting,cheng2018intrinsic} from which the error numbers are indeed close to $0$ (see Tab.~\ref{tab:sintel_image_split}, they are multiplied by 100).


LapPyrNet~\cite{cheng2018intrinsic} performs in general the second best. It employs several loss functions such as joint bilateral filtering loss, VGG perceptual loss, \etc. %Particularly, the VGG loss makes use of a VGG-Net pretrained on ImageNet and results in very low DSSIM. 
Notwithstanding, our results show that the proposed simple spectral loss (Tab.~\ref{tab:sintel_scene_split}, only $\mathcal L_{\text{spec}}$) is as effective as these multiple losses .

Qualitative illustrations are
presented in Fig.~\ref{figure:mpi_scenesplit} and Fig.~\ref{figure:mpi_imagesplit} where in particular
the low-frequency part of the sky and high frequency details
of the person's face illustrate the improved prediction thanks to the spectral structure.

\input{tab_mpi_imagesplit.tex}
\input{fig-mpi-imagesplit.tex}
%
%
\subsection{Results on MIT Intrinsic}
\label{subsec:mit}

% The MIT dataset contains $110$ real world images for training, which is not sufficient for most CNN-based methods; additional data are often employed to help the training~\cite{shi2017learning,narihira2015direct,cheng2018intrinsic,cgintrinsic}; FFI-Net is instead trained with the MIT Intrinsic only. 

% Prior works use various combinations of the performance metrics, but
% we include all of them for completeness to Tab.~\ref{tab:mit} and Tab.~\ref{tab:mit_b}.
For MIT Intrinsic, \cite{lettry2018darn,fan2018revisiting,cheng2018intrinsic} report si-MSE and si-LMSE and while \cite{cgintrinsic, baslamisli2018cnn, li2018learning} report MSE, LMSE and DSSIM. We include both in Tab.~\ref{tab:mit} and~\ref{tab:mit_b} for comprehensive comparison.

With si-MSE and si-LMSE (Tab.~\ref{tab:mit}), FFI-Net outperforms the competing
deep learning methods. The traditional method SIRFS~\cite{barron2015shape} has 
%FFT-Net achieves si-MSE 0.71, 0.79 and 0.75 on albeod, shading and their average, while~\cite{barron2015shape} obtains 0.64, 0.98 and 0.81, correspondingly. 
slightly better si-MSE for albedo and total si-LMSE. It uses a prior that is particularly suitable for the MIT Intrinsic images; we notice its clear inferiority over others on MPI-Sintel in Tab.~\ref{tab:sintel_image_split}. 
MIT is a rather small dataset and is therefore
 often trained with additional datasets~\cite{shi2017learning,narihira2015direct} while FFI-Net only trains on MIT. 

%Initiated by a series of works~\cite{narihira2015direct,fan2018revisiting,cheng2018intrinsic}, we emphasize on scale-invariant metrics as reported in Tab.\ref{tab:mit}.



%IntriNet~\cite{baslamisli2018joint} significantly outperforms others on nearly all the metrics. Accordingly, it has its own evaluation protocol while we follows~\cite{}. We download the released official results from RetiNet~\cite{baslamisli2018cnn} \footnote{https://ivi.fnwi.uva.nl/cv/retinet} evaluate them with our protocol; we report the results as xx in Table xx, which are much lower than ours (shown in Tab.\ref{tab:mit}). 

%More supporting visual comparison with \cite{baslamisli2018cnn} can be found in supplement.
%we find it less consistent compared to Tab.~\ref{tab:mit}. For example, RetiNet~\cite{baslamisli2018cnn} reports surprisingly better results than CG~\cite{cgintrinsic} and Ma \etal~\cite{ma2018single}, while the latter two were more up-to-date. 

% \miaojing{I am not sure how to write this, as FFI-Net is inferior to [25], and clearly worse than [4], while Yanlin suggests that [4]'s numbers are not reliable after looking at its graphic results, which are super bad. Maybe @Matas or @Joni can take care of this para ?   }

\input{tab_mit_A.tex}
\input{tab_mit_B.tex}



\input{fig-mit.tex}
% \input{fig-mit2.tex}
%
%

We also provide results in MSE, LMSE, and DSSIM in Tab.~\ref{tab:mit_b}.
FFI-Net performs in general better than latest works \eg~\cite{ma2018single,cgintrinsic,liu2020cvpr}. 
%\cite{cgintrinsic} uses additional synthetic data (CGI) in its training;  
Notice that it appears that
%does not report DSSIM and
the LMSE in \cite{ma2018single} is computed using a different window size, thus its two numbers (italic) in LMSE are not comparable to others. 
%Despite our good results on MSE, LMSE, DSSIM, 
%We would like to emphasize our results on the scale-invariant measures in Tab.\ref{tab:mit}, as initiated by a series of works~\cite{narihira2015direct,fan2018revisiting,cheng2018intrinsic}.  

\subsection{Results on IIW} 
\label{subsec:iiw}
%\input{fig-iiw.tex}

The IIW dataset differs substantially from MPI-Sintel and
MIT Intrinsic in its ground truth. IIW does not have dense pixel-wise ground truth with physical grounds, but only sparse pair-wise annotations of points
in each image. Therefore the losses relying on dense prediction, e.g., GAN discriminator loss/VGG loss,
in ~\cite{cheng2018intrinsic,lettry2018darn,ma2018single,shi2017learning} cannot apply. That also prevents using our spectral
loss and sub-branch losses. For this experiment, our proposed
loss functions were replaced with the WHDR loss used in~\cite{fan2018revisiting}. Our network structure remains encoded with spectral weights. 

The WHDR scores are shown in Tab.~\ref{table:iiw}. FFI-Net, despite being disabled with spectral banding and loss, still achieves competitive WHDR score $15.81$ among the state-of-the-arts~\cite{cgintrinsic,fan2018revisiting,zhou2019glosh}. The best performance by~\cite{fan2018revisiting} can be partly explained by its tailored domain filter that flattens albedo prediction. While ~\cite{cgintrinsic} and \cite{zhou2019glosh} use additional datasets (\eg CGI, SAW, SUNCG) along with IIW for training augmentation. 
%augmented annotations for training.


%only trained on original IIW, we still obtain $16.31$ WHDR using a default-setting architecture. Note that 
\input{tab-iiw.tex}

%\input{fig-iiw-withsota.tex}
\input{fig-iiw.tex}

\input{fig-wospecloss.tex}

%
%
\subsection{Ablation Study}
\label{secsec:results_spectralweights}
% We conduct the ablation study on MPI-Sintel in the scene split setting.  
\para{Spectral Bands.}
Tab.~\ref{tab:sintel_scene_split} demonstrates that adding more spectral bands ($M$) consistently improves the results. We use $M=5$ as a trade-off between efficiency and accuracy.
%\miaojing{In addition, we also conduct another experiment by replacing the spectral banding with the spatial scale decomposition proposed in ~\cite{cheng2018intrinsic}, the spectral loss is disabled in this circumstance while the spectral residual block remains. 
%Notice in order to still apply spectral loss in this variant, we need to specifically transform multiple spatial bands into Fourier domain. 
%The result (w/ $B_\text{spat}$) is clearly lower than FFI-Net, and is also inferior to that without spectral loss but with spectral banding (w/o $\mathcal L_{\text{spec}}$ (M =5, $R_{\text{spec}}$)). This shows spectral banding provides better frequency steering in the scale space compared to~\cite{cheng2018intrinsic}; also it enables the usage of spectral loss.  }
%, as  $M>5$ increases much complexity but rewards with marginal improvement.
%\miaojing{it would be better if we have M=7 result}.  
It is worth mentioning that using a single spectral band already outperforms the state-of-the-arts in si-MSE and si-LMSE. We believe this is due to the spectral encoding of residual blocks and the spectral loss.



% \begin{table}
% \setlength{\tabcolsep}{4pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1} % Default value: 1
% \centering
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{l | rrr | rrr | rrr}
% \toprule
%  &
% \multicolumn{3}{c}{si-MSE$\times10^{2}$} & \multicolumn{3}{c}{si-LMSE$\times10^{2}$} & \multicolumn{3}{c}{DSSIM$\times10^{2}$}\\
% & A & S & avg & A & S & avg & A & S & avg\\
% \midrule
% spat-1 & 1.52 & 1.67 & 1.60&~0.91 & 1.14 & 1.02 & 11.04 & 11.69 & 11.37\\
% spat-3 & 1.41 &  1.44 & 1.42~& 0.82 & 0.93 & 0.88 &  10.59 & 9.95  & 10.27\\
% spat-5 & 1.50 &  1.50 & 1.50~& 0.91 & 0.92 & 0.91 &  10.25 & 9.78  & 10.01\\
% \midrule
% spec-1 & 1.35 &  1.36 & 1.35 & 0.82 & 0.82 & 0.82 &  10.43 & 10.84 & 10.63\\
% spec-3 & 1.24 &  1.16 & 1.20 & 0.75 & 0.75 & 0.75 &  9.59 & 8.85  & 9.22\\
% spec-5 & {1.19} &  {1.16} & {1.18} & {0.73} & {0.73} & {0.73} &  9.03 & {8.60} & {8.82} \\
% \bottomrule
% \end{tabular}}
% \caption{Influence of spectral band number $M \in \{1,3,5\}$ and
% of the  spectral (spec) vs. spatial (spat) residual blocks. Results on MPI-Sintel (scene-split). }
% \label{tab:sintel_scene_split_weightsvsweights} 
% \vspace{-0mm}
% \end{table}
\medskip 

\para{Spatial vs Spectral Residual Blocks.}
% The convolutional filters in the spectral residual blocks are encoded with complex values, which differs from the original spatial residual blocks~\cite{he2015deep}.
Tab.~\ref{tab:sintel_scene_split} shows using spectral residual blocks performs significantly better than the spatial residual blocks ($R_\text{spat}$ v.s. $R_\text{spec}$). 
%Particularly, the result using spectral residual blocks in only one band ($M=1$) already outperforms that using spatial residual block with five bands ($M=5$). 
Fig.~\ref{figure:without_spectralloss} shows using spectral residual blocks significantly accelerates the convergence rate (3x - 5x) and improves the accuracy. 
%Further discussion about the compactness of the spectral encoding will be presented below in the session Network parameters.  
% We guess the reason lies in: spectral encodes filters are considerably sparser, thereby reducing the redundancy that appears in spatial domain representations. It results in a much faster (3x - 5x) convergence rate compared to the net using spatial coding; more importantly, it provides the
% Adam optimizer with more meaningful axis-aligned directions which eventually results in better test performance.
% THIS IS NOT EASY TO UNDERSTAND:
%We guess the reason lies in: spectral coding axis-aligns the search space to %more meaningful directions.

\medskip 
%
\para{Spectral Loss.} Tab.~\ref{tab:sintel_scene_split} reports the results of FFI-Net without spectral loss (w/o $\mathcal L_\text{spec}$): the performance is inferior to FFI-Net on the metrics si-LMSE and DSSIM but remains the same on si-MSE. Unsurprisingly, si-MSE defines the pixel-wise loss while si-LMSE and DSSIM consider the window-wise correlations.
The results demonstrate the effectiveness of spectral loss on the global similarity between the intrinsic prediction and the corresponding ground truth. Moreover, we point out that FFI-Net (only $\mathcal L_\text{spec}$) already outperforms the state-of-the-arts~\cite{cheng2018intrinsic,lettry2018darn,fan2018revisiting} on si-MSE and si-LMSE. %Some ablation study in MIT Intrinsic is presented in Tab.~\ref{tab:mit}



\begin{table}[t]
\setlength{\tabcolsep}{1.5pt}
\centering
\small
\begin{tabular}{l ccccc}
\hline
{Method}& Fan \cite{fan2018revisiting} & Darn \cite{lettry2018darn} & Lap \cite{cheng2018intrinsic} & CGI~\cite{cgintrinsic} & FFI-Net \cr
\hline
Parameters(Train) ~ & 2.80 &  17.97 & 138 & 7.7 & 0.75 \cr
Parameters(Test) ~ & 2.80 &  0.74 & 0.94 & 7.7 & 0.75  \cr
\hline
\vspace{-5mm}
\end{tabular}
\caption{Network parameter numbers displayed in million-scale. The training parameters for \cite{lettry2018darn} and \cite{cheng2018intrinsic} includes that of the GAN discriminator and the VGG classifier, respectively.
}
\label{tab:parameter_and_time}. 
%\vspace{-5mm}
\end{table}

\medskip 
\para{Network parameters and inference time. }
Tab.~\ref{tab:parameter_and_time} profiles the network parameter number of FFI-Net. 
It generally needs less parameters compared to the others, which use extra guidance network~\cite{fan2018revisiting}, adversarial network~\cite{lettry2018darn}, VGGNet~\cite{cheng2018intrinsic} and U-Net~\cite{cgintrinsic} for training. %The spectral encoding needs fewer parameters with the same effective dimensionality. 
%We also report the real inference time among 
\miaojing{As for inference time, we reproduced~\cite{fan2018revisiting,cheng2018intrinsic} with the same GPU (GTX 1080) as ours, it is $\sim$100 ms for~\cite{fan2018revisiting}, $\sim$70 ms for~\cite{cheng2018intrinsic} and $\sim$42 ms for FFI-Net.}

%as it uses real and imaginary parts.
% The parameter number for test is the same with training, making it the lightest network compared to other representative works. 



% \input{fig-iiw.tex}
% \input{tab-iiw.tex}



==> WACV2021_ Fourier-Camera Ready/fig-iiw-supple.tex <==
\begin{figure*}[htb]
  \centering
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    
    

        \vspace{-1mm}
        \\  
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881-albedo.png}& 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881-shading.png}
  
          \vspace{-1mm}
        \\  
        %% 3rd row
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122-albedo.png}& 
                \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122-shading.png}
                
%           \vspace{-1mm}
%         \\  
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_img.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_bell_A.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_bell_S.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_zhou_A.jpg} & 
% 		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_zhou_S.jpg} &         
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_cg_A.jpg}  & 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_cg_S.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735-albedo.png}& 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735-shading.png}
        
        
                  \vspace{-1mm}
        \\  
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54-albedo.png}& 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54-shading.png}

                  \vspace{-1mm}
        \\  
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155-albedo.png}& 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155-shading.png}


%         \vspace{-1mm}
%         \\  
%         %% 3rd row
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/img/118514.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/bell/118514-r.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/bell/118514-s.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/118514-r.jpg} & 
% 		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/118514-s.jpg} &         
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/118514-r.jpg}  & 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/118514-s.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/118514-albedo.png}& 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/118514-shading.png}
        
    
         \vspace{-1mm}
        \\                       
        {\scriptsize Image} & {\scriptsize Bell~\cite{bell2014intrinsic} ($A$)}  & {\scriptsize Bell~\cite{bell2014intrinsic}($S$)} & {\scriptsize Zhou~\cite{zhou2015learning} ($A$)}  & {\scriptsize Zhou \cite{zhou2015learning} ($S$)}  & {\scriptsize CGI \cite{cgintrinsic} ($A$)} & {\scriptsize CGI \cite{cgintrinsic} ($S$)}   &  {\scriptsize FFI-Net ($A$)} & {\scriptsize FFI-Net ($S$)}
    \end{tabular}  
  \caption{ Qualitative comparisons of (A)lebdo and (S)hading on IIW.
    % Our predictions show significant improvements compared to
    % state-of-the-art algorithms (bell~\etal ~\cite{bell2014intrinsic}
    % and zhou~\etal~\cite{zhou2015learning}). 
    % In particular, our
    % predicted shading channels include significantly less surface
    % texture in several challenging
    % settings.
    } \label{fig:iiw} 
\end{figure*}

==> WACV2021_ Fourier-Camera Ready/fig-iiw-withsota.tex <==
% \setlength{\tabcolsep}{0.1pt}
% \renewcommand{\arraystretch}{1}
\begin{figure*}
\centering
%\begin{tabular}{ccccccc}
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155.png}& 
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_am_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_am_our.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155-albedo.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_shading_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_shading_our.png} &
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155-shading.png} \\
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940.png}& 
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_am_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_am.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940-albedo.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_shading_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_shading.png} &
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940-shading.png} \\
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54.png}& 
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_am_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_am.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54-albedo.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_shading_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_shading.png} &
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54-shading.png} \\
Images & Li \cite{BigTimeLi18} (A) & \cite{yu2019inverserendernet} (A) & FFI-Net (A) & Li \cite{BigTimeLi18} (S) &  \cite{yu2019inverserendernet} (S) & FFI-Net (S)\\
\end{tabular}
    \vspace{-0.2cm}
    \caption{Qualitative comparison with latest SoTAs for IIW. Second column to forth column are reflectance predictions from Li~\cite{BigTimeLi18}, InverseRenderNet~\cite{yu2019inverserendernet} and ours.}
     \label{fig:iiw-with-sota}
\end{figure*}

==> WACV2021_ Fourier-Camera Ready/fig-iiw.tex <==

\begin{figure*}[ht]
  \centering
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        \includegraphics[width=0.11\textwidth, height=0.07\textwidth]{comp_iiw/img/5735.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/5735-r.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/5735-s.jpg}  &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/5735-r.jpg}  & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/5735-s.jpg}  &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/5735-r.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/5735-s.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/5735-r.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/5735-s.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/5735-albedo.png}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/5735-shading.png}  
        
        \vspace{-1mm}
        \\  
        %% second row 
       % \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/img/26760.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/26760-r.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/26760-s.jpg} &
    %    \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/26760-r.jpg} & 
	%	\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/26760-s.jpg}  &         
     %   \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/26760-r.jpg}  & 
      %  \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/26760-s.jpg}  & 
        
      %  \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/26760-r.jpg}  & 
      %  \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/26760-s.jpg}  & 
      %  \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/26760-albedo.png}  & 
      %  \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/26760-shading.png}  
        
      %  \vspace{-1mm}
      %  \\  
        %% 3rd row
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/img/102887.jpg} &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/102887-r.jpg} &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/102887-s.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/102887-r.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/102887-s.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/102887-r.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/102887-s.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/102887-r.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/102887-s.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/102887-albedo.png}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/102887-shading.png}
        
        \vspace{-1mm}
        \\          

        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/img/72329.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/72329-r.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/72329-s.jpg}  &
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/72329-r.jpg}  & 
		%\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/72329-s.jpg} &         
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/72329-r.jpg}  & 
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/72329-s2.jpg}  &
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/72329-r.jpg}  & 
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/72329-s.jpg}  &
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/72329-albedo.png}   &
        %\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/72329-shading.png}  
        
        
        
        %  \vspace{-1mm}
        % \\     

        % \includegraphics[width=0.11\textwidth]{comp_iiw/img/118514.jpg}  &
        % % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/118514-r.jpg}  &
        % % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/118514-s.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/zhou/118514-r.jpg} & 
        % \includegraphics[width=0.11\textwidth]{comp_iiw/zhou/118514-s.jpg} &         
        % \includegraphics[width=0.11\textwidth]{comp_iiw/cg/118514-r.jpg} & 
        % \includegraphics[width=0.11\textwidth]{comp_iiw/cg/118514-s.jpg} &
        %         \includegraphics[width=0.11\textwidth]{comp_iiw/fan/118514-r.jpg} & 
        % \includegraphics[width=0.11\textwidth]{comp_iiw/fan/118514-s.jpg} &
        %         \includegraphics[width=0.11\textwidth]{comp_iiw/cg/118514-r.jpg} & 
        % \includegraphics[width=0.11\textwidth]{comp_iiw/cg/118514-s.jpg} 
        
        
      %  \vspace{-1mm}
      %  \\

      %% 10th row
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/img/101121.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/101121-r.jpg}  &
        % \includegraphics[width=0.11\textwidth]{comp_iiw/bell/101121-s.jpg}  &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/101121-r.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/101121-s.jpg}  &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/101121-r.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/101121-s.jpg}  &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/101121-r.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/fan/101121-s.jpg}  &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/101121-albedo.png}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/101121-shading.png}
         \vspace{-1mm}
        \\                       
        {\scriptsize Image} & {\scriptsize Zhou~\cite{zhou2015learning} ($A$)}  & {\scriptsize Zhou \cite{zhou2015learning} ($S$)}  & {\scriptsize CGI \cite{cgintrinsic} ($A$)} & {\scriptsize CGI \cite{cgintrinsic} ($S$)}   & {\scriptsize Fan \cite{fan2018revisiting} ($A$)} & {\scriptsize Fan \cite{fan2018revisiting} ($S$)} & {\scriptsize FFI-Net ($A$)} & {\scriptsize FFI-Net ($S$)}
    \end{tabular}  
  \caption{ Qualitative comparisons of (A)lbedo and (S)hading on IIW. Results of our FFI-Net are visually very similar to the best performing results~\cite{fan2018revisiting}. 
    % Our predictions show significant improvements compared to
    % state-of-the-art algorithms (bell~\etal ~\cite{bell2014intrinsic}
    % and zhou~\etal~\cite{zhou2015learning}). 
    % In particular, our
    % predicted shading channels include significantly less surface
    % texture in several challenging
    % settings.
    } \label{fig:iiw} 
\end{figure*}

==> WACV2021_ Fourier-Camera Ready/fig-mit-supple.tex <==
%\setlength{\tabcolsep}{0.1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[htp]
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c c ccccc}
\vspace{-0.5mm}
\!\!\includegraphics[width=1.4cm]{comp_MIT/turtle_input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo_di.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo_fan.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_label_albedo.jpg}\cr
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading_di.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading_fan.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading.jpg}\\

\vspace{-0.5mm}

\!\!\includegraphics[width=1.4cm]{comp_MIT/deer_input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo_di.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo_fan.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_label_albedo.jpg}
\\
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_shading_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_shading_di.jpg}
&\includegraphics[width=1.4cm,,height=1.215cm]{comp_MIT/deer_predict_shading_fan.jpg}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/deer_predict_shading.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_shading.jpg}\\

%\vspace{-0.75mm}
%
%\includegraphics[width=1.4cm]{pear-1-input.jpg}
%
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo-Shijian.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo-DI.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo.jpg}
%&\includegraphics[width=1.4cm]{pear-1-labelA.jpg}
%
%&\includegraphics[width=1.4cm]{pear-1-predict-shading-Shijian.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-shading-DI.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-shading.jpg}
%&\includegraphics[width=1.4cm]{pear-1-labelS.jpg}\\

%\vspace{-0.75mm}
%
%\includegraphics[width=1.4cm]{turtle-1-input.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo-Shijian.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo-DI.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-labelA.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading-Shijian.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading-DI.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-labelS.jpg}\\

\vspace{-0.5mm}

\small{Input} & & \small{Shi \emph{et al.} \cite{shi2017learning}} & \small{DI \cite{narihira2015direct}} & \small{Fan \textit{et al.} \cite{fan2018revisiting}} & \small{FFI-Net} & \small{Ground Truth}\\

% \vspace{-0.6mm}

% &\multicolumn{4}{ c }{\small{Albedo}} & \multicolumn{4}{ c }{\small{Shading}}\\
\end{tabular}}

\end{center}
\vspace{-2mm}
\caption{Sample  (A)lbedo and (S)hading on MIT Intrinsic. 
%Only trained on MIT itself, our method can produce visually-pleasing output, similiar to Fan \textit{et al.} \cite{fan2018revisiting}
}
\label{figure:mit-supple}
\vspace{-0mm}
\end{figure}


==> WACV2021_ Fourier-Camera Ready/fig-mit.tex <==
%\setlength{\tabcolsep}{0.1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[htp]
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c c ccccc}
\vspace{-0.5mm}
\!\!\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-predict-albedo-Shijian.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-predict-albedo-DI.jpg}
&\includegraphics[width=1.4cm,height=1.003cm]{comp_MIT/raccoon-1-predict-albedo-Fan.jpg}
&\includegraphics[width=1.4cm,,height=1.003cm]{comp_MIT/raccoon-1-predict-albedo.png}
&\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-labelA-mark.jpg}\cr
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-predict-shading-Shijian.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-predict-shading-DI.jpg}
&\includegraphics[width=1.4cm,,height=1.003cm]{comp_MIT/raccoon-1-predict-shading-Fan.jpg}
&\includegraphics[width=1.4cm,height=1.003cm]{comp_MIT/raccoon-1-predict-shading.png}
&\includegraphics[width=1.4cm]{comp_MIT/raccoon-1-labelS-mark.jpg}\\

\vspace{-0.5mm}

\!\!\includegraphics[width=1.4cm]{comp_MIT/paper2-1-input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm]{comp_MIT/paper2-1-predict-albedo-Shijian.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/paper2-1-predict-albedo-DI.jpg}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/paper2-1-predict-albedo-Fan.jpg}
&\includegraphics[width=1.4cm,,height=1.215cm]{comp_MIT/paper2-1-predict-albedo.png}
&\includegraphics[width=1.4cm]{comp_MIT/paper2-1-labelA.jpg}\\
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm]{comp_MIT/paper2-1-predict-shading-Shijian.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/paper2-1-predict-shading-DI.jpg}
&\includegraphics[width=1.4cm,,height=1.215cm]{comp_MIT/paper2-1-predict-shading-Fan.jpg}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/paper2-1-predict-shading.png}
&\includegraphics[width=1.4cm]{comp_MIT/paper2-1-labelS.jpg}\\

%\vspace{-0.75mm}
%
%\includegraphics[width=1.4cm]{pear-1-input.jpg}
%
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo-Shijian.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo-DI.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo.jpg}
%&\includegraphics[width=1.4cm]{pear-1-labelA.jpg}
%
%&\includegraphics[width=1.4cm]{pear-1-predict-shading-Shijian.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-shading-DI.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-shading.jpg}
%&\includegraphics[width=1.4cm]{pear-1-labelS.jpg}\\

%\vspace{-0.75mm}
%
%\includegraphics[width=1.4cm]{turtle-1-input.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo-Shijian.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo-DI.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-labelA.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading-Shijian.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading-DI.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-labelS.jpg}\\

\vspace{-0.5mm}

\small{Input} & & \small{Shi \emph{et al.} \cite{shi2017learning}} & \small{DI \cite{narihira2015direct}} & \small{Fan \textit{et al.} \cite{fan2018revisiting}} & \small{FFI-Net} & \small{Ground Truth}\\

% \vspace{-0.6mm}

% &\multicolumn{4}{ c }{\small{Albedo}} & \multicolumn{4}{ c }{\small{Shading}}\\
\end{tabular}}

\end{center}
\vspace{-2mm}
\caption{Sample (A)lbedo and (S)hading on MIT Intrinsic. FFI-Net performs better for object details (top), as well as for the overall appearance (bottom). 
%Only trained on MIT itself, our method can produce visually-pleasing output, similiar to Fan \textit{et al.} \cite{fan2018revisiting}
}
%\vspace{-2mm}
\label{figure:mit}
\end{figure}


==> WACV2021_ Fourier-Camera Ready/fig-mit2.tex <==
%\setlength{\tabcolsep}{0.1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[htp]
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c c ccccc}
\vspace{-0.5mm}
\!\!\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_no_imf_turtle_albedo.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_yes_imf_turtle_albedo.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/retinet_turtle_albedo.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_predict_albedo.jpg}
&\includegraphics[width=1.4cm,,height=1cm]{comp_MIT/turtle_label_albedo.jpg}
\cr
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_no_imf_turtle_shading.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_yes_imf_turtle_shading.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/retinet_turtle_shading.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_predict_shading.jpg}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_label_shading.jpg}
\\

\vspace{-0.5mm}

\!\!\includegraphics[width=1.4cm]{comp_MIT/paper2-1-input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_no_imf_paper2_albedo.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_yes_imf_paper2_albedo.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/retinet_paper2_albedo.png}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/paper2-1-predict-albedo.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT/paper2-1-labelA.jpg}\\
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_no_imf_paper2_shading.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_yes_imf_paper2_shading.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/retinet_paper2_shading.png}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/paper2-1-predict-shading.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT/paper2-1-labelS.jpg}\\

\vspace{-0.5mm}

\small{Input} & & IntriNet  & IntriNet  & Retinet & \small{FFI-Net} & \small{Ground Truth}\\
 & & w/o imf\cite{baslamisli2018cnn} &  w/ imf\cite{baslamisli2018cnn} & \cite{baslamisli2018cnn} &  & \\

% \vspace{-0.6mm}

% &\multicolumn{4}{ c }{\small{Albedo}} & \multicolumn{4}{ c }{\small{Shading}}\\
\end{tabular}}

\end{center}
\vspace{-2mm}
\caption{Sample  (A)lbedo and (S)hading on MIT Intrinsic. Comparison with different versions in~\cite{baslamisli2018cnn}. Results of~\cite{baslamisli2018cnn} are downloaded from their project webpage.
%Only trained on MIT itself, our method can produce visually-pleasing output, similiar to Fan \textit{et al.} \cite{fan2018revisiting}
}
\vspace{-3mm}
\label{figure:mit2}
\end{figure}


==> WACV2021_ Fourier-Camera Ready/fig-mpi-imagesplit-supple.tex <==
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[t]
\begin{center}

%\begin{tabular}{cccc}
%
%%\vspace{-0.75mm}
%%\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}} \\
%%
%%\vspace{-0.75mm}
%%\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}\\
%%
%%\vspace{-0.75mm}
%%\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}\\
%%
%%\vspace{-0.75mm}
%%{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}\\
%%&\scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} & \scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} \\
%
%\vspace{-0.75mm}
%&\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.5\height}{\rotatebox{90}{\scriptsize{\textbf{Albedo}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.3\height}{\rotatebox{90}{\scriptsize{\textbf{Shading}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}}}\\
%
%\end{tabular}

\begin{tabular}{ccc}

\vspace{-0.75mm}
\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}
&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-input.jpg}}
\\
& (A) & (S) \\
% \vspace{-0.75mm}
% \raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Lee~\cite{lee2012estimation}}}}}
% &{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-lee.jpg}}}
% &{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-lee.jpg}}}
% \\

\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Barron~\cite{barron2015shape}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-barron.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-barron.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Chen~\cite{chen2013simple}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-chen.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-chen.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-di.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-di.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-fan.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-fan.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Lap\cite{cheng2018intrinsic}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-lap.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-lap.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-fft.png}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-fft.png}}}
\\

\vspace{-0.75mm}
{\rotatebox{90}{\scriptsize{{Ground Truth}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-label-albedo-mark.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-label-shading-mark.jpg}}}
\\
\vspace{-5mm}

\end{tabular}


\end{center}
\vspace{-2.5mm}
\caption{More Examples of (A)lbedo and (S)hading predictions on MPI-Sintel (image split). %FFI-Net performs well in difficult parts, \eg hair bunchesa and  cast shadows.
}
\label{figure:mpi_imagesplit_supple}
\vspace{-3mm}
\end{figure}

%Compared to state-of-the-art method MSCR \cite{DI2015}, we show much sharper effects and better performance.


==> WACV2021_ Fourier-Camera Ready/fig-mpi-imagesplit.tex <==
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[t]
\begin{center}

%\begin{tabular}{cccc}
%
%%\vspace{-0.75mm}
%%\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}} \\
%%
%%\vspace{-0.75mm}
%%\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}\\
%%
%%\vspace{-0.75mm}
%%\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}\\
%%
%%\vspace{-0.75mm}
%%{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}\\
%%&\scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} & \scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} \\
%
%\vspace{-0.75mm}
%&\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.5\height}{\rotatebox{90}{\scriptsize{\textbf{Albedo}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.3\height}{\rotatebox{90}{\scriptsize{\textbf{Shading}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}}}\\
%
%\end{tabular}


\begin{tabular}{ccc}

\vspace{-0.75mm}
\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}
&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-input.jpg}}
\\
& (A) & (S) \\
\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Lee~\cite{lee2012estimation}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-lee.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-lee.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Barron~\cite{barron2015shape}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-barron.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-barron.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Chen~\cite{chen2013simple}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-chen.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-chen.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-di.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-di.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-fan.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-fan.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Lap\cite{cheng2018intrinsic}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-lap.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-lap.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-albedo-fft.png}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-predict-shading-fft.png}}}
\\

\vspace{-0.75mm}
{\rotatebox{90}{\scriptsize{{Ground Truth}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-label-albedo-mark.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/1-label-shading-mark.jpg}}}
\\
\vspace{-5mm}

\end{tabular}


\end{center}
\vspace{-5mm}
\caption{Examples of (A)lbedo and (S)hading predictions on MPI-Sintel (image split). FFI-Net performs well in difficult parts, \eg person fingers, faces (red arrows).
% \miaojing{Barron remove ! DI can be replaced with some ECCV work}
}
\label{figure:mpi_imagesplit}
\vspace{-2mm}
\end{figure}

%Compared to state-of-the-art method MSCR \cite{DI2015}, we show much sharper effects and better performance.


==> WACV2021_ Fourier-Camera Ready/fig-mpi-scenesplit.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1}
\begin{figure}[t]
\begin{center}

%\begin{tabular}{cccc}
%
%%\vspace{-0.75mm}
%%\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}} \\
%%
%%\vspace{-0.75mm}
%%\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}\\
%%
%%\vspace{-0.75mm}
%%\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}\\
%%
%%\vspace{-0.75mm}
%%{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}\\
%%&\scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} & \scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} \\
%
%\vspace{-0.75mm}
%&\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.5\height}{\rotatebox{90}{\scriptsize{\textbf{Albedo}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.3\height}{\rotatebox{90}{\scriptsize{\textbf{Shading}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}}}\\
%
%\end{tabular}


\begin{tabular}{ccc}

\vspace{-0.75mm}
\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}
&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-input.jpg}}
\\
& (A) & (S) \\
\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-predict-albedo-DI.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-predict-shading-DI.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-predict-albedo-fan.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-predict-shading-fan.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-predict-albedo.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-predict-shading.jpg}}}
\\

\vspace{-0.75mm}
{\rotatebox{90}{\scriptsize{{Ground Truth}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-label-albedo-mark.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/alley_2_frame_0047-label-shading-mark.jpg}}}
\\

\end{tabular}

\end{center}
\caption{Examples on the MPI-Sintel (scene split). We emphasize the ability of FFI-Net of shadow removal (\eg sky - red arrows) in the unseen scene compared to others. 
}
\label{figure:mpi_scenesplit}
%\vspace{-5mm}
\end{figure}

%Compared to state-of-the-art method MSCR \cite{DI2015}, we show much sharper effects and better performance.


==> WACV2021_ Fourier-Camera Ready/fig-mpi-scensplit-supple.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1}
\begin{figure}
\begin{center}
\vspace{-3mm}
\begin{tabular}{ccc}

%\vspace{-0.75mm}
%\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-input.jpg}}\\& (A) & (S) \\
%\vspace{-0.75mm}
%\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-albedo-MSCR.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-shading-MSCR.jpg}}}\\

%\vspace{-0.75mm} \raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-albedo-fan.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-shading-fan.jpg}}}\\

%\vspace{-0.75mm}
%\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-albedo.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-shading.jpg}}}\\

%\vspace{-0.75mm}
%{\rotatebox{90}{\scriptsize{{Ground Truth}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-label-albedo.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-label-shading.jpg}}}\vspace{5mm}\\

\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}
&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-input.jpg}}
\\
& (A) & (S) \\
\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-albedo-MSCR.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-shading-MSCR.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-albedo-fan.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-shading-fan.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-albedo.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-shading.jpg}}}
\\

\vspace{-0.75mm}
{\rotatebox{90}{\scriptsize{{Ground Truth}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-label-albedo-mark.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-label-shading-mark.jpg}}}
\\


\vspace{-5mm}

\end{tabular}

\end{center}
\vspace{-2.5mm}
\caption{Examples on the MPI-Sintel dataset (scene split). }
\label{figure:mpi_scenesplit_supple}
%\vspace{-3mm}
\end{figure}

%Compared to state-of-the-art method MSCR \cite{DI2015}, we show much sharper effects and better performance.


==> WACV2021_ Fourier-Camera Ready/fig-wospecloss.tex <==
\begin{figure}
\begin{center}

% \begin{tabular}{cc}

% \hspace{-4.5ex}
% \begin{tabular}{ccc}
% \vspace{-0.75mm}
% %\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{albedo}}}}
% &\multicolumn{2}{c}{\includegraphics[width=55mm,height=50mm]{img/converge_MPI.png}}
% \end{tabular}

% & 

% \hspace{-4.5ex}
% \begin{tabular}{ccc}
% \raisebox{.9\height}{\rotatebox{90}{\scriptsize{{albedo}}}}
% &\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp_wospecloss/gt_specloss.jpg}}
% \\
% \vspace{-0.75mm}
% \raisebox{.9\height}{\rotatebox{90}{\scriptsize{{w/o $\mathcal{L}_s$}}}}
% &\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp_wospecloss/wo_specloss.jpg}}
% \\
% \vspace{-0.75mm}
% \raisebox{.9\height}{\rotatebox{90}{\scriptsize{{with $\mathcal{L}_s$}}}}
% &\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp_wospecloss/with_specloss.jpg}}
% \\
% \vspace{-2mm}
% \end{tabular}
% \end{tabular}

\includegraphics[width=\linewidth]{img/converge_MPI.png}
\end{center}
\caption{
Network training convergence for the proposed spectral (red) and the conventional (blue) residual blocks. 
% Right: ground truth albedo (top), prediction without
% the spectral loss (center) and with the spectral loss (bottom). Results on MPI-Sintel (scene-split).
%\miaojing{I'll remove this figure for space if necessary but simply talking in text}
}
%\vspace{-3mm}
\label{figure:without_spectralloss}
\end{figure}

==> WACV2021_ Fourier-Camera Ready/fig_architecture.tex <==
\begin{figure*}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{img/fft_architecture.png}
\vspace{-5mm}
\caption{
%Overview of FFI-Net. Different to a fully-spatial deep net for intrinsic image decomposition, FFI-Net contains:
%(a)~$\mathscr{F}$ and $\mathscr{F}^{-1}$ layers that convert spatial space representations to the spectral space using the Fast Fourier Transform (FFT) and its inverse (Sec. \ref{subsec:fft}) ; (b) \textit{spectral residual blocks} where residual block weights are coded in Fourier domain (Sec. \ref{subsec:ournetwork}); (c)
% \textit{spectral banding} that learns the multi-path structures with ground truth of different spectral bands (Sec. \ref{subsec:spectralbanding}); \textit{spectral banding} that splits a spectral map into several bands and associates them with ground truth of specific frequency bands.
% (d) \textit{spectral loss} which measures global error between the prediction and ground truth in the Fourier domain (Sec. \ref{subsection:spectralloss}).
% (a) and (b) are firstly adopted while (c) and (d) are novelly proposed in intrinsic decomposition.   We only show the red-channel spectral map for simplicity.
Overview of FFI-Net. Different from other deep intrinsic image decomposition architectures, FFI-Net offers several new modules:
(a) $\mathscr{F}$ and $\mathscr{F}^{-1}$ layers that convert between spatial and spectral domains using
the Fast Fourier Transform (FFT) and its inverse (Sec. \ref{subsec:fft}) ; (b) \textit{spectral residual blocks} where residual block weights are parametrized in the spectral domain (Sec. \ref{subsec:ournetwork});
(c)
% \textit{spectral banding} that learns the multi-path structures with ground truth of different spectral bands (Sec. \ref{subsec:spectralbanding});
\miaojing{\textit{spectral banding} that splits a spectral map into $M$ (e.g. M = 3) overlapped (low-pass) spectral bands at the beginning of the network and associates $M$ non-overlapped spectral bands of the image in both spatial and spectral domain as ground truth by the end of the network.}
(d) \textit{spectral loss} which measures global error between the prediction and ground truth in the spectral domain (Sec. \ref{subsection:spectralloss}).}
%(a) and (b) are firstly adopted while (c) and (d) are novelly proposed in intrinsic decomposition.
\label{fig:architecture}
\end{center}
\vspace{-5mm}
\end{figure*}


==> WACV2021_ Fourier-Camera Ready/introduction.tex <==
\section{Introduction}
Intrinsic image decomposition refers to the problem of separating an image $\mathcal{I}$ into its
\emph{albedo} and \emph{shading}~\cite{barrow1978recovering}, where \emph{albedo} models the diffuse reflection of the scene materials and 
\emph{shading} represents the lighting and scene geometry.
We adopt the common assumption that the problem can be simplified to the per-pixel image formation
$\mathcal{I}=\mathcal{A}\cdot\mathcal{S}$ where $\mathcal A$ and $\mathcal S$ are the
albedo and shading, respectively. 
Factorization of $\mathcal{I}$ into $\mathcal{A}$ and $\mathcal{S}$ is ill-posed.
Early work tackled the factorization by applying constraints and priors which connect the properties of
materials and lighting in the physical world with the gradient and color changes in images~\cite{land1971lightness,horn1974determining}; however,
even the sophisticated physical modelling can
not fully cover the  complex optical interactions among materials,
light sources, and object/scene geometry. % (flat or strong edge, corner) 
%(point or parallel) 
Intrinsic image decomposition is an open and challenging problem {\em per~se}, but it can also benefit many other vision problems, \textit{e.g.}, {semantic segmentation}~\cite{baslamisli2018joint}, {depth estimation}~\cite{kim2016unified}, and {color constancy}~\cite{barron2015shape}. 


% \begin{figure}[h]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{img/gray_spectral_pooling_banding_reduced.png}
% \caption{
% Spectral cropping in spatial (top) and frequency domains (3rd row) vs. the proposed Spectral banding (2nd and bottom rows). Unlike in spectral cropping, spectral frequency bands are orthogonal, without  redundancy.\textcolor{red}{Joni: Is this figure strong enough for the first page?\miaojing{this figur will be replaced by fig2}}
% % In the spectral cropping the same information is repeated while in the spectral banding the frequency bands are orthogonal and therefore provide richer features with the same number of weights.
% %We can get an impression that: Pooling in spectral domain works as spatial smoothing filter, while banding as spatial edge filter.
% \label{fig:intro_fftbanding}}
% \end{center}
% \end{figure} 

Traditional approaches for intrinsic image decomposition are surveyed in~\cite{barron2015shape}, while recent state-of-the-art performance has been achieved with image-to-image translation networks as in~\cite{narihira2015direct,fan2018revisiting,cheng2018intrinsic,lettry2018darn,li2018learning,liu2020cvpr}. The mean squared error (MSE) loss is typically employed in the network training to enforce pixel-wise similarity between the predicted and ground truth albedo and shading~\cite{fan2018revisiting,lettry2018darn,cheng2018intrinsic}.
The MSE loss does not consider correlations between image pixels.  
Extra loss terms such as loss for the learnable domain filter~\cite{fan2018revisiting}, perceptual
loss~\cite{cheng2018intrinsic} and generative adversarial loss \cite{lettry2018darn}, are often added to enforce global similarities between predictions and ground truth. 
Proposed models also exploit a multi-path structure in their networks to separate the prediction into different levels of details~\cite{cheng2018intrinsic} or contexts~\cite{li2018learning,fan2018revisiting}. 


%These networks share two design principles that we willintroduce their spectral counterparts in this work. First, the pixel-wise loss (\eg MSE) or other special losses (\eg VGG perceptual loss~\cite{johnson2016eccv} or generative adversarial loss) are employed to enforce similarity between the predicted and ground truth albedo and shading~\cite{fan2018revisiting,lettry2018darn,cheng2018intrinsic}.Second, the models often exploit a multi-path structure to separate the prediction to different levels of details~\cite{cheng2018intrinsic} or contexts~\cite{li2018learning,fan2018revisiting}. 
%For example, 
%Cheng \etal \cite{cheng2018intrinsic} proposed a Laplacian pyramid of the %output albedo and shading and build a hierarchical network for that. Li %\etal \cite{li2018learning} separated the intrinsic shading estimation %into global illumination estimation and non-chromatic shading estimation. 
%Since MSE does not consider correlations between image pixels, 
%some special loss terms have been considered for training:
%the loss for the learnable domain filter~\cite{fan2018revisiting}, VGG %perceptual
%loss~\cite{cheng2018intrinsic} and generative adversarial loss %\cite{lettry2018darn}.  

% In this work, we show that network training in the spectral (Fourier)
% domain improves image-to-image translation for intrinsic image
% decomposition. In particular,  we propose a
% {\em Fast Fourier Intrinsic Network} (FFI-Net)
% which measure global feature correlation more effectively than the
% special loss terms in the previous works~\cite{cheng2018intrinsic,lettry2018darn}. In addition,
% we replace the multi-path structure of the previous
% works~\cite{li2018learning,fan2018revisiting,lettry2018darn,cheng2018intrinsic} with spectral banding that enables continuous tuning of network features. Moreover, we also found that gradient learning
% of complex-valued network weights in the spectral space provide better accuracy
% than traditional stochastic gradient descent in the spatial domain
% real-valued weights.

In this work, we propose a \textbf{F}ast \textbf{F}ourier \textbf{I}ntrinsic \textbf{Net}work (FFI-Net)  for intrinsic image decomposition. 
The network design focuses on the multi-path architecture and loss function, as were intensively exploited in recent works~\cite{li2018learning,fan2018revisiting,lettry2018darn,cheng2018intrinsic}, but differs substantially from the prior arts since no published intrinsic decomposition method operates in the spectral domain.
The intuition is based on  the observation that published approaches
~\cite{fan2018revisiting,cheng2018intrinsic} often separate the predictions of structure and details into different scales, implicitly performing 
operations that are indeed best understood in the spectral domain. 
Image details, \eg fine edges, are naturally reflected in the high-frequency part;
on the other hand, image structures such as flattened color patches are usually reflected in the low-frequency part. 
%
Despite the frequency interpretation behind the previous works, their models were optimized in the spatial domain. 
Thus if the intrinsic image decomposition task is solved in the spectral domain, we might expect, 
and this is confirmed by our experiments, the optimization of the network to be more efficient and effective, as in the classification task ~\cite{rippel2015spectral}. 
Furthermore, since each pixel in the spectral domain is a complex-weighted sum over the image space,  a pixel-wise loss on the spectral map thus can straightforwardly enforce a global similarity between the prediction and ground truth in the spatial domain.     
%- FFI-Net - which is trained using a spectral loss term in addition to the spatial loss terms and adopts spectral banding to build a multi-path architecture, as in the prior art~\cite{li2018learning,fan2018revisiting,lettry2018darn,cheng2018intrinsic}. The motivation of spectral banding is that the multi-path architecture addressing levels of details (gradients) can be better interpreted in the Fourier domain. 
%The spectral loss is introduced to measure global feature correlation since each
%bin in Fourier domain is a complex-valued descriptor over the whole spatial image. Moreover, we empirically find that spectral parameterization of the network weight allows better accuracy for intrinsic image decomposition, as we expect, similar to image classification~\cite{rippel2015spectral}. 

% 1, It inspired us that some published approaches~\cite{fan2018revisiting,cheng2018intrinsic} often separate the predictions of structure and details into different scales, implicitly performing operations that can be better understood in the Fourier domain. 
% Image details, \eg fine edges, are naturally reflected in the high-frequency part, while image structures such as flattened color patches are usually reflected in the low-frequency part. 
%
% 2, In addition to the frequency interpretation, the models of the previous works were optimized in the spatial domain. Thus, if the intrinsic image decomposition task is solved in the spectral domain, we might expect, and this is confirmed by our experiments, the optimization of the network to be simpler and faster, as in the classification work ~\cite{rippel2015spectral}. 
%
% 3, Furthermore, each pixel in the Fourier domain is a complex-weighted sum over the image space. A pixel-wise loss on the spectral map thus straightforwardly reflects a global measure between the prediction and ground truth in the spatial domain.     

\para{Contributions.}
We propose a novel network architecture for intrinsic image decomposition where the following spectral operations and structures replace their
spatial domain counterparts used in the prior works:
%
\begin{compactitem}
% \item We propose complex-valued (odd-even signal decomposition) spectral
% layers~\cite{guberman2016complex,rippel2015spectral} for the problem of intrinsic image decomposition; principally we parameterize the widely-used residual block~\cite{he2015deep} with spectral CNN weights and adapt conjugate symmetry of complex numbers to accept arbitrary input size. 
%
% \item We propose a \textit{spectral banding} technique in the frequency domain which splits input image into several frequency bands and feed them together into the network to build a multiscale (multi-frequency) model that enables more optimal scale steering of features than discrete scales in the previous works (see Fig.~\ref{fig:intro_fftbanding}).
\item \textit{Spectral banding} splits the input image into several frequency bands, therefore allowing multi-path training and inference (see Fig.~\ref{fig:architecture}).

\item \textit{Spectral loss} provides a global error measure on the similarity between the predicted $\mathcal{A}$/$\mathcal{S}$ and the corresponding ground truth, effectively augmenting the pixel-wise loss.

\item \textit{Spectral residual block} encodes original residual block with  spectral weights, thus obtaining faster convergence to a lower error.

\end{compactitem}


To the best of our knowledge, FFI-Net is the first to address intrinsic decomposition in the Fourier domain.
Our experiments with three intrinsic image datasets (MPI-Sintel, MIL Intrinsic and IIW) demonstrate state-of-the-art accuracy for FFI-Net. 
%On the third dataset, IIW, 
%which provides only a sparse ground truth, FFI-Net performs competitively to prior
%art even if the techniques relying on dense ground truth (\eg the spectral loss) need to be turned off. 



%Despite the  
%plainly formulated as $\textit{I} \approx \textit{A} \odot \textit{S}$ 

%With continuous research efforts put on image disentanglement tasks, , one core task, \textit{intrinsic image decomposition}, has strong correlation with other tasks and still remains a open task.  , where we denote $A$ as \textit{albedo} (), $S$ as \textit{shading}, which covers all photometric effects triggered by environment illumination, cast shallows, captured geometry. 
% \sout{Depth prior is hidden in $shading$ \cite{kong2015intrinsic}. More complex image formation models, considering specular refletion, are introduced and explored by \cite{shi2017learning}. } 
% \miaojing{they are not related to your work unless you want to solve the depth problem or the more complex decomposition problem.Add something else to further describe the A and S. } 

%\miaojing{
% Try to wrote the below para in the following way: Intrinsic image decomposition is not easy because it is an ill-posed problem, requiring a mapping from $n$ known variables (image $I$) to $n^2$ ($2n$ ??) unknown variables (albedo $A$ and shading $S$). To solve this problem, traditional approaches reply on the prior constraints to infer the material/lighting change from the gradient/color change in images\cite{land1971lightness,horn1974determining}. The image decomposition task is usually addressed in several sub-problems corresponding to different priors. Despite the sophisticated physical reasoning behind each prior, the complex optical interaction among materials (common or nameless), geometry (flat or strong edge, corner) and light source (point or parallel) makes it still hard to jointly model xxx every prior in different scenarios. 

% Due to the recent advent of deep features\cite{xx}, modern approaches instead employs the convolutional neural networks (CNN) to directly conduct an image-to-image transformation\cite{fan2018revisiting,cheng2018intrinsic}. A specific mapping is learnt in the network to enforce a pixel-wise similarity between the predicted map and ground truth. The task is not decomposed based on certain priors, but is expanded into multi-scale in scale space. For example, Fan et al.~\cite{fan2018revisiting} introduce a double-column network with one column responsible for direct intrinsic generation while the other one provide guidance on the edges, xx etc. Cheng~\cite{cheng2018intrinsic} further exploit the scale space and propose a multi-branch of details decompisition blabl. Because CNNs are particularly good at predicting locally rather than globally, apart from the pixel-wise loss, researchers also try to introduce some losses to address the visual similarity between prediction and ground truth in a global sense such that Fan et al. domain filter , cheng perceptual loss, lettry et al gan loss.  

% In this work, we revisit the spectral representation in CNN\cite{xx}. We notice that in the previous works, the edge information indeed naturally reflects in the high-frequency part in the spectral domain, while the color information naturally reflects in the low-frequency part. Despite the frequency interpretation behind, the previous networks are still optimized in the space domain. If we transform the whole image decomposition task into spectral domain, the search space would be perfectly match xxx blabla some works from \cite{xx} about the search space. Furthermore, in the spectral domain, each pixel  indeed represent the global information in the space domain, a pixel-wise loss on the spectral map natually enforce a globa similarity between the prediction and the GT.     

% Building upon the observation above, in this work , we propose a spectral xxx cnn to xxx, we offer several new elements in this archiecture: xxxx
%}



% To learn better mapping from input image to albedo and shading, we find main-stream works are evolving in two directions.  The first is that a lot of efforts are put into decomposing the task into sub problems. Traditional methods \cite{barron2015shape,chen2013simple} search for feasible solutions, meeting natural prior constraints in material reflectance, shape and casting illumination, simultaneously. Retinex theory \cite{land1971lightness}, geometric change or cast shadows triggers abrupt image gradient in shading image. \textit{Horn} \cite{horn1974determining} attributes large image gradient to material change and small gradient to spatial-varying lighting.
% Supervised CNN-methods \cite{narihira2015direct, fan2018revisiting, lettry2018darn} uses hourglass-like network with skip connections to learn pixel and edge information. Unsupervised CNN method \cite{li2018learning} splits the task of shading estimation into global illumination estimation and non-chromatic shading map. \cite{cheng2018intrinsic} proposed a hierarchy network mapping Level-of-Detail of input to that of output. The other direction is that as mean square loss is local and generate artifacts, more-global loss is introduced to learn high-level description. Edge-preserving domain filter is adopted by \cite{fan2018revisiting} to flatten albedo. \cite{lettry2018darn} imports global constraint by adding adversarial loss. 


% Traditional methods \cite{barron2015shape,chen2013simple} constrains searching space based on natural prior on the material reflectance, shape and casting illumination. For instance, stated in Retinex theory \cite{land1971lightness}, geometric change or cast shadows triggers abrupt image gradient in shading image. \textit{Horn} \cite{horn1974determining} attributes large image gradient to material change and small gradient to spatial-varying lighting. Another branch is data-driven learning-based method \cite{kong2015intrinsic, fan2018revisiting, lettry2018darn}, with or without using CNN. Concerning image gradient, we can retreat these methods as ones learning to classify whether a region of gradient belongs to albedo or shading, which learns better local minima than handcraft priors.

% In this work, we put our efforts on exploring these two directions. Inspired by \textit{spectral pooling} \cite{rippel2015spectral}, we treat large-value spatial gradient as high-frequency point in spectral domain and wonder: \textit{can we split the problem into orthogonal sub-problems in spectral domain? can we compute a global loss in spectral domain?}.




==> WACV2021_ Fourier-Camera Ready/methodology.tex <==
\section{Fast Fourier Intrinsic Network}\label{sec:method}
Before presenting the building blocks of FFI-Net, we review the properties of the Discrete Fourier Transform.
%We would like to thank the reviewers for their comments, which are helping us to improve the quality of our work. Our responses follow.
% \miaojing{I would organze this section this way: 1. preliminary. it includes sect.3.2 as well as some key techniques in the spectral paper like spectral pooling and conjugate symmetry constraints (sec3.4). 2. Network Architecture. Sec3.1 gives an overview picture of our network design and some overview idea of spectral banding and spectral loss. Say that we will detail the two techniques below. 3. Spectral banding (Sec. 3.3) 4. Spectral loss; 5. network training.
% Part of Sec.3.4 about your adaption can be put into item 2 Overview.
% Sec. 3.5 is boring, you can split it into item 2 and 5.
% P.S. Fig.2 is very weird. You should present a whole architecture with data flow explicitly drawn. Cureently, it looks like our network takes image and fft and then ifft, then goes with original conv, but it is not like that! Does it ? }

% \begin{figure*}[h]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{img/fft_architecture.png}
% \caption{The proposed Deep Intrinsic Image Decomposition architecture. {\em Spectral banding}~\cite{rippel2015spectral} provides multiscale processing in the frequency
% domain. {\em Spectral residual blocks} are similar to the conventional residual blocks~\cite{he2015deep} but their weights are optimized in the Fourier (spectral)
% domain instead of the spatial domain. {\em Spectral banding} guarantees that the
% parallel network branches steer to features on certain frequency (scale) bands.
% Finally, the band-wise features are summed to minimize the {\em spectral loss} term.
% The main operations are
% the discrete Fourier transform (DFT) $\mathscr{F}$ and its inverse (IDFT)
% $\mathscr{F}^{-1}$ that are both performed efficiently using the Fast Fourier
% Transform (FFT/IFFT).
% %For better visual effect, we only show spectral map of red channel out of three and all spectral maps (except for the first row) are element-wise added by $128$. 
% \label{fig:architecture}}
% \end{center}
% \end{figure*} 


%
% \subsection{Architecture Overview}
% The proposed Deep Fourier Intrinsic Image Decomposition architecture
% is shown in Figure~\ref{fig:architecture}. The architecture consists
% of the following elements: {\em spectral pooling}, {\em spectral residual blocks},
% {\em spectral banding} and {\em spectral loss}. In the following,
% the spectral pooling from~\cite{rippel2015spectral} is first
% revisited and then the three elements proposed in this work are described in
% more details.

%
%
\subsection{Preliminaries}
\label{subsec:fft}

% \textcolor{red}{I think that the material in this subsection should be divided under 3.2 Preliminaries (Fourier transform and its properties used in this work) and 3.3 Spectral Pooling (revisited from Rippel et al.)}

%
\para{The Discrete Fourier Transform (DFT).} 
% It is the equivalent of the continuous Fourier in the discrete space~\cite{give a reference here}.
%Given an input image ${I \in \mathbb{C}^{H \times W}}$ with height $H$ and width $W$, the DFT %produces its representation in spectral domain: 
For a discrete 2D image $I(h,w) = I \in \mathbb{R}^{H \times W}$ where
$h=0,\ldots,H-1$ and $w=0,\ldots, W-1$, the
Fourier domain representation is computed by 
%
%\vspace{-5mm}
\begin{align}
& \mathscr{F}(I)_{nm} = \frac{1}{\sqrt{HW}}\sum_{h=0}^{H-1} \sum_{w=0}^{W-1} I(h,w) e^{-2\pi i(\frac{nh}{H} + \frac{mw}{W})}\qquad \notag \\
& \forall n\in\{0,\ldots, H-1\}, \forall m\in\{0,\ldots, W-1\}\;.  
\end{align}
%
% The important properties of Fourier transform used in this work are~\cite{Bracewell-1999}:
% {\em symmetry}, {\em Parseval's theorem} and {\em XX}; and in the following
% the properties are briefly described.
The DFT is linear and unitary and $I$ can be restored using the inverse DFT given by ${\mathscr{F}^{-1}(I)=\mathscr{F}(I)^*}$, which is the conjugate of the transform itself. 

%
\vspace{\medskipamount}
\para{Properties of DFT for CNN.}\\ 
%For efficient and effective implementation of CNN with Fourier transform layers, the following theorems and properties are exploited: {\em convolution theorem}, {\em Fourier transform differentation} and {\em conjugate symmetry}.
\noindent\emph{Convolution theorem:}
Convolution in the spatial domain is equal to the element-wise product in the spectral domain: 
%
\begin{align}
\mathscr{F}(x*f) = \mathscr{F}(x)\odot\mathscr{F}(f),
\end{align}
%
where we denote by $x$ and $f$ two spatial signals (\eg images), $*$ and $\odot$ the operators of the convolution and the Hadamard product, respectively. %This powerful property is leveraged to speed-up the training of CNNs in~\cite{mathieu2013fast,lavin2016fast}.
% Till now, we have introduced common sense about FFT, in following we will discuss other benefits FFT can bring to our task.
DFT can be implemented using the Fast Fourier Transform (FFT), 
%which takes advantage of the recursive structure of the Fourier transform to accelerate DFT. FFT manages to 
which reduces the complexity of DFT from $\mathcal{O}((HW)^{2})$ to $\mathcal{O}(HW \log (HW))$.
%\textcolor{red}{This complexity is for 1-D signal, we should give it to an image}

\medskip
\noindent\emph{DFT differentiation:} For CNN backpropagation algorithms, the gradients must be
propagated through Fourier transform layers. Suppose a DFT layer $\mathscr{F}$ maps a real-valued input $x \in \mathbb{R}^{H \times W}$ to $z \in \mathbb{C}^{H \times W}$, and $\frac{\partial{\mathcal L}}{\partial{z}}$ is the gradient of loss $\mathcal L$ w.r.t $z$; Since both $\mathscr{F}$ and $\mathscr{F}^{-1}$ are unitary, the back-propagation through $\mathscr{F}$ and $\mathscr{F}^{-1}$ can be written as 
\begin{align}
\frac{\partial \mathcal L}{\partial{x}} = \mathscr{F}^{-1}\left(\frac{\partial \mathcal L}{\partial{z}}\right)\;,
~~~
\frac{\partial \mathcal L}{\partial{z}} = \mathscr{F}\left(\frac{\partial \mathcal L}{\partial{x}}\right)\;.
\label{eq:gradient}
\end{align}
% Similarly, the back-propagation of the inverse FFT (IFFT) is:
% \begin{align}
% \frac{\partial L}{\partial{Z}} = \mathscr{F}\left(\frac{\partial L}{\partial{X}}\right)\;.
% \end{align}
%This differentiable property makes $\mathscr{F}$ and $\mathscr{F}^{-1}$ portable layers in CNN.



%\begin{figure}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{img/conjugate.png}
%\caption{The four possible symmetry patterns of different input dimensionality (odd/even width and height). 
% From left to right: (odd, odd), (even, odd), (odd, even), (even, even). 
%{Orange}: real-valued components; {Blue}: no constraints; {Gray}: values fixed by conjugate symmetry. See also ~\cite{rippel2015spectral}. 
%\label{fig:conjugate}}
%\vspace{-3mm}
%\end{center}
%\end{figure} 

%

%\noindent\emph{Conjugate symmetry constraint:} To guarantee that the restored image $\mathscr{F}^{-1}(z)$ is real-valued, the {conjugate symmetry} condition must be retained in $z$
%\begin{align}
%\label{eq:conjugatesym}
%z_{nm} =z^*_{{(H - n)\,\textrm{mod} H, (W - m)\,\textrm{mod} W}}\qquad \notag \\
%\forall n\in\{0,\ldots, H-1\}, \forall m\in\{0,\ldots, W-1\}\;.
%\end{align}
% \miaojing{I do not understand this sentence but try to put an interpretable sentence here to explain }
% Specifically, when $Z_{yx}$ and $Z_{(-y)x}$ coincide modulo $M$, both elements are real-valued. 
%The DC component $Z_{00}$ is complex conjugate to itself. %Given a real input, its $\mathscr{F}$ will necessarily meet this. 
%The conjugate symmetry constraint will be adapted and verified later in our network design (Sec.~\ref{subsec:ournetwork}). %when we use $\mathscr{F}^{-1}$ in CNN.
%For image classification task, the input size is usually fixed, \eg a square~\cite{rippel2015spectral}. For image-to-image translation task, the input size can be arbitrary; hence, we offer all four possible conjugate symmetry patterns in Fig.~\ref{fig:conjugate} with respect to the odd/even dimensionalities of the input's height and width ($H$, $W$).
%(odd, odd), (even, odd), (odd,even), and (even, even). 
%Referring to Eq.~\ref{eq:conjugatesym}: the blue pixels have no constraints, while the grey pixels are of fixed values by conjugate symmetry; orange pixels are with real values.
%By replacing $H$ and $W$ with any odd/even values (integers) in Fig~\ref{fig:conjugate}, we can adapt the constraints to arbitrary input size. 





%such that the the   It is realized by directly dropping a predefined high-frequency part of spectrum and doing $\mathscr{F}^{-1}$ on the remaining spectrum, which gives an efficient aliasing-free downsampling method.

%layers We first give a definition of a spectral conv layer: As opposed to an ordinary CNN with each filter~${w\in\mathbb{R}^{H\times W}}$, a CNN with spectral CNN weights has each filter ~${\theta \in\mathbb{C}^{H\times W}}$. We can get the spatial representation of the filter using $\mathscr{F}^{-1}(\theta)$. In back propagation, once a conv layer with spectral weights receive gradient $ \frac{\partial L}{\partial{X}}$ of the global loss \textit{w.r.t.} this layer (this layer outputs $X$), the real-valued gradients are transformed to the frequency domain $\mathscr{F}(\frac{\partial L}{\partial{X}})$ to update the spectral weights $\theta$.
% Hereafter, we can connect spectral conv layer with other common layers, \textit{e.g.} adding Relu, Batch Normalization. 
 
%Large-kernel CNN weights can be encoded in spectral domain (complex value), which provides an appealing basis for learning object-level representation for image classification \cite{rippel2015spectral}. However, this strategy has not been validated on small kernels (\eg size $3$) and dense-mapping tasks \textit{e.g.} intrinsic image decomposition.
 
%To learn residual (frequency spectrum disparity in our task) functions in a deep CNN, we propose spectral residual block, which is shown in  Figure \ref{fig:spectralresidualblock}. In all experiments, our spectral residual block consists of $2$ conv layer with $32$ channels and $3\times3$ filter size.
%The only difference compared to the original residual block is the weight encoding way. 
 


%such that the the   It is realized by directly dropping a predefined high-frequency part of spectrum and doing $\mathscr{F}^{-1}$ on the remaining spectrum, which gives an efficient aliasing-free downsampling method.


\subsection{The Network Architecture}
\label{subsec:ournetwork} 
Our network architecture is built upon the preliminary discussion about DFT and extended to the intrinsic image decomposition task with several new components (see Fig.~\ref{fig:architecture}). The input image $I$ is first transformed into the spectral representation $\mathscr{F}({I})$. Spectral banding (Sec.~\ref{subsec:spectralbanding}) is applied afterwards to crop the spectral feature map of $\mathscr{F}({I})$ into $M$ overlapped (low-pass) sub-representations. DC component is centered in the spectral feature map in Fig.~\ref{fig:architecture}. 
% The $M$ spectral maps are transformed back to the spatial domain via $\mathscr{F}^{-1}$  to account for the implementation of non-linear transform i.e. ReLu in the spatial domain. 
% We feed each sub representation into $N$ consecutive spectral residual blocks afterwards, two streams are split at the point of the $\frac{N}{2}$-th block to infer both the albedo and shading. 
The $M$ spectral bands are transformed back to the spatial domain via $\mathscr{F}^{-1}$ as input to feed into $N$ consecutive spectral residual blocks, respectively (Fig.~\ref{fig:spectralresidualblock} and Sec.~\ref{subsec:residual}). \miaojing{Spectral residual blocks parametrize the conv weights in the spectral domain for optimization yet their input and output are in the spatial domain. The outputs of the $M$ subbranches are transformed to the spectral domain, ground truth in two domains are associated both before and after the transformation. The $M$ ground truth are generated via the spectral banding that is different from previous: it produces a series of non-overlapped bands similar to the Laplacian pyramid (Sec.~\ref{subsec:spectralbanding}). The $M$ spectral maps predicted in the network are summed up to create a complete spectral map of the image and further converted back to the spatial domain; again, ground truth are associated both in the spectral and spatial domain on the complete image.  
The loss function between the ground truth and network predictions are introduced in the spatial and spectral domain, respectively (Sec.~\ref{subsection:spectralloss} and~\ref{subsec:loss}): the spatial loss employs the commonly used pixel-wise MSE in the original images and their gradient maps~\cite{fan2018revisiting,lettry2018darn} (Sec.~\ref{subsec:loss}); the spectral loss also utilizes pixel-wise MSE loss but on the spectral maps, which provides an additional global constraint on the intrinsic prediction (Sec.~\ref{subsection:spectralloss}).}
Notice that, to infer both the albedo and shading simultaneously, after the $\frac{N}{2}$-th block of each subbranch we split it into two streams for albedo and shading, respectively.  

Below we present the spectral residual block, spectral banding, and spectral loss. 


%, which contains non-linear transform, \ie ReLu. Till our knowledge, ReLu has not been implemented in spectral domain. 

% To allow the summation of subbranches to form a complete map prediction, we propose a spectral banding technique (Sec.\ref{subsec:spectralbanding}) to separate the ground truth into $M$ sub representations with unique frequency bands. We associate them separately to each subbranch for the network training.  
%Below we first introduce the technique of spectral encoding in residual block, and then detail the spectral banding and spectral loss.


% Rippel \textit{et al.} \cite{rippel2015spectral} firstly learn the filters of CNN in frequency domain and prove its success on image classification task. In other words, the CNN weights are FFT-transformed to the spectral domain and stored in complex value. Here we adopt this weight encoding strategy and explore its potential advantage on dense-mapping tasks \textit{e.g.} intrinsic image decomposition.
\subsection{Spectral Residual Block} \label{subsec:residual}
Residual blocks~\cite{he2015deep} are widely applied for intrinsic image decomposition~\cite{fan2018revisiting,lettry2018darn}. Inspired by~\cite{rippel2015spectral}, we expect that spectral encoding of residual blocks can help solve the intrinsic decomposition task.
As shown in Fig.~\ref{fig:spectralresidualblock}, given a two-conv layer residual block, \miaojing{its input and output are in the spatial domain but the conv weights are parametrized in the spectral domain. These weights need to be converted back to the spatial domain when convolving with the input. This reparametrization does
not alter the underlying model, it provides an appropriate domain for parameter optimization, as the frequency basis captures typical filter structure well.
As suggested in~\cite{rippel2015spectral}, spectral encoding of the network results in more compact convolutional filters with more meaningful axis-aligned directions for optimization. 
In the experiment we demonstrate that residual blocks with spectral weights boost the performance.}
%A network with spectral weights is trained similar to a standard
%network with equivalent structure, 

\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{img/spectral_block.png}
\caption{ 
% \miaojing{if we want to keep it , it has to be bigger and more importantly, we should signify with F($\cdot$) (text is optional) inside the block of weight layer and spectral weight layer to show what is really different}
Illustration of the original (left) residual block and proposed spectral residual block (right). $\theta$ denotes the kernel weights of convolutional filters. 
%The kernel weight $\theta$ is originally in the spatial domain and real-valued (left) while in the right $\theta$ is in the spectral domain and complex-valued.
\label{fig:spectralresidualblock}
}
\vspace{-5mm}
\end{center}
\end{figure} 
%

%we convert the conv weights ($\theta$) to the spectral domain for weights optimization via the FFT cuDNN implementation. 

%They need to be converted back afterwards as there is no spectral implementation of ReLu in cuDNN. Extra computational cost for $\mathscr{F}$ and $\mathscr{F}^{-1}$ to adapt for ReLu is negligible thanks to the efficient cuDNN implementation.
%Notice the 
%A network with spectral weights is trained similar to a standard
%network with equivalent structure, 


% Convolution is performed in the spatial domain which benefits from efficient
% GPU implementations.

%\emph{Spectral residual block.} We adopt a 2-layer residual block shown in Fig.~\ref{fig:spectralresidualblock}(a) which consists of convolutions, ReLu and skip connections. Following~\cite{rippel2015spectral}, we parametrize the two convolutional layers with spectral weights. ReLu remains in the spatial domain, the network forward and backward in the residual block require two extra passes of  $\mathscr{F}$ and $\mathscr{F}^{-1}$ executions on the two convolutional layers as compared to the original residual block (see Fig.~\ref{fig:spectralresidualblock}(b)). 
%The extra operation time is negligible thanks to an efficient FFT cuDNN implementation. In return, it results in more compact convolutional filters with more meaningful axis-aligned directions for optimization. 
% \miaojing{this is not very interesting, considering remove this sentence - $>$ }
%The spectral CNN weights in \cite{rippel2015spectral} are used with different sized kernels, but in Sec.~\ref{secsec:results_spectralweights} we demonstrate that by only using small kernels in a residual block, it is still helpful. 

%\emph{Conjugate Symmetry constraint on arbitrary size.} 
%The conjugate symmetry constraint applied in~\cite{rippel2015spectral} is only for square input in image classification task. We adapt it on arbitrary input size for image-to-image translation tasks. 
%The size of an arbitrary input falls into four categories with respect to the odd/even dimensionalities of its height and width ($H$, $W$): (odd, odd), (even, odd), (odd,even), and (even, even). We offer the four conjugate symmetry patterns in Fig.~\ref{fig:conjugate}, where we illustrate $H$ and $W$ as either 7 or 8; the DC component lies at the top left corner.
%According to Eq.~(\ref{eq:conjugatesym}): the blue pixels have no constraints, while the grey pixels are of fixed values by conjugate symmetry; orange pixels are with real-valuedness constraint. By replacing $H$ and $W$ with any odd/even values (integers) in Fig~\ref{fig:conjugate}, we can adapt the constraints to arbitrary input size.  

%and thus works as a strong backbone network for intrinsic image task. 
%Here we note that these spectral bands may be not zeros but very small values in the center in real inference phase. 
%The final output is obtained by inverse transform the summed map. 
%To build FFI-Net and make it work for intrinsic image decomposition, we we principally %present two adaptions (spectral residual block and arbitrary-size conjugate symmetry %constraints) and two new components (spectral banding and spectral loss) in the following.



\subsection{Spectral Banding}
\label{subsec:spectralbanding}


% Spectral banding is to let each network subbranch learn a sub representation corresponding to a specific frequency band of the original image. 
Inspired by the multi-path structure in~\cite{cheng2018intrinsic}, which conducts scale space separation of the albedo/shading image, we instead perform a spectral domain separation, which provides more fine-grained control over frequency. 
The spectral banding is formulated as:
\begin{align}
\label{eq:spectralbanding}
    z_{nm}=
    \begin{cases}
      \mathscr{F}(x)_{nm}, & \text{if}\ n \in [N_l,N_u], m \in [M_l,M_u] \\
      0, & \text{otherwise} 
    \end{cases}
\end{align}

In a spectral map, values between $N_l$ and $N_u$ in $x$-axis, $M_l$ and $M_u$ in $y$-axis are kept. If $N_l$ and $M_l$ are always zeros, \textit{spectral banding} works like a smoothing filter. %rather an edge filter, 
%which is also conceptualized as spectral cropping in previous work~\cite{rippel2015spectral}. 
\miaojing{We apply this special case of spectral banding ($N_l$ and $M_l$ are zeros while $N_u$ and $M_u$ are increased over bands) at the beginning of the network to split the input into overlapped bands (see Fig.~\ref{fig:architecture} before the spectral residual blocks).} If $N_l$ and $M_l$ are non-zeros, \miaojing{we can separate the spectral map into multiple bands where the upper bounds ($N_u$, $M_u$) of a current band are taken as the lower bounds ($N_l$, $M_l$) of its adjacent band with higher frequency.} When we apply the inverse FFT to these spectral bands, they look like image Laplacian pyramid with different levels of details~\cite{burt1983tc,liu2020acmmm} (see Fig.~\ref{fig:architecture} after the spectral residual blocks). In the network, we generate $M$ of these non-overlapped spectral bands from the ground truth to associate at the end of each subbranch. In this way, the subbranch output can be summed together to recover the final prediction (we call it \textit{summing spectral bands} in Fig.~\ref{fig:architecture}). 

In practice, we can provide a specific range of $nm$ for $z_{nm}=0$ in Eq.~\ref{eq:spectralbanding}, where the spatial transform of a spectral band can be of adjustable size related to the predefined range. This makes spectral banding flexible with any input and output size in a fully-convolutional neural network. Notice the {level-of-detail} exploited in~\cite{cheng2018intrinsic} is obtained by applying the fix-sized Gaussian kernel in the spatial domain, while spectral banding retrieves the level-of-detail in the spectral domain explicitly and more effectively; \miaojing{Most importantly, our spectral banding enables the effective usage of another new component, spectral loss, as below.   }
% We generate $M$ spectral bands and their edge maps from the original image
% ; they are utilized as ground truth for each network subbranch separately.    

%Note that the \textit{spectral cropping} proposed by~\cite{rippel2015spectral} can be seen as a special case of \textit{spectral banding} when $N_d$ and $M_d$ are equal to zeros. 
% In practice, they serve differently:  \textit{spectral banding} works like an edge filter, while \textit{spectral cropping} a smoothing filter. 
%In practice, when $N_d$ and $M_d$ are zeros, \textit{spectral banding} works like a smoothing filter, rather an edge filter.



% \vspace{\medskipamount}
% \para{Spectral Banding.}
% % \miaojing {copy and re paraphrase some sentences from \cite{rippel2015spectral}.}
% Spectral banding (spectral cropping) was originally proposed for dimensionality reduction~\cite{rippel2015spectral,zhang2017weakly}. 
% It is implemented by cropping the high-frequency part from the spectral representation; $\mathscr{F}^{-1}$ is applied on the remaining components to restore the representation in the space domain. A 2D image can be down-sampled into low-resolutions in this way. Spectral banding is justified by
% the prior works that use more traditional scale-space discretization (Laplacian pyramid)~\cite{fan2018revisiting,cheng2018intrinsic}.
% The scale-space is non-optimal as the scales (frequencies) are manually
% selected while spectral banding provides more continuous frequency
% adjustment.




\subsection{Spectral Loss}
\label{subsection:spectralloss}
%We sum the subbranch outputs from the network to predict the final albedo/shading. 
Loss functions are defined in both the spectral and spatial domains, here we first detail the spectral loss: since each pixel in the spectral domain is a weighted sum of the whole image in the spatial domain, a pixel-wise loss defined on the spectral representation spontaneously enforces a global similarity between the spatial prediction and the ground truth. Inspired by the global loss applied  in~\cite{lettry2018darn,fan2018revisiting,cheng2018intrinsic}, we propose a spectral loss defined in the spectral domain:  
\begin{align}\label{eq:spectralloss}
\mathcal{L}_s(x,\hat{x}) = \|\mathcal{M}(\mathscr{F}(x))-\mathcal{M}(\mathscr{F}(\hat{x}))\|_2^2 
%\\+\|\Im(\mathscr{F}(x)) - \Im(\mathscr{F}(\hat{x}))\|_2^2, \notag
\end{align}
where $\hat{x}$ and $x$ denote the predicted and ground truth albedo/shading in the spatial domain, respectively. 
$\mathcal M$ is defined as an operator to take the magnitude of a complex value, $\mathcal{M}(\mathscr{F}(x)) = |\mathscr{F}(x)|$
%, where $\mathcal R$ and $\mathcal I$ takes the real and imaginary part of the complex value, respectively. 
We only use the magnitude part as it contains information of the image geometric structure in the spatial domain while discarding the phase part as ``invisible" \miaojing{(see ~\cite{R.fisher,dip_book}). This also empirically gives us benefits whilst minimizing the error over the phase part does not. Notice if we minimize the squared error for the real and imaginary components, since $\mathscr{F}$ is a linear transform, it will be identical to minimizing the squared error in the spatial domain, as specified below. }
%The back-propagation is:
%\begin{align}\label{eq:finalloss}
%\frac{\partial \mathcal L_s}{\partial{x}} = 
% \mathscr{F}^{-1}( 2\mathcal M(\mathscr{F}(x)) %- 2\mathcal M(\mathscr{F}(\hat{x})) ),
%\end{align}
%where the term inside $\mathscr{F}^{-1}$ is real and always meets the symmetry constraint such that after $\mathscr{F}^{-1}$ the loss gradient $\frac{\partial \mathcal L_s}{\partial{x}}$ is also real.

%We note that in prior works~\cite{fan2018revisiting,lettry2018darn,cheng2018intrinsic} the global losses in the spatial domain usually come with additional branch in the network.
\miaojing{In FFI-Net, spectral losses are directly applied pixel-wise on the $M$ spectral outputs of the network as well as on  their summation.  }
%the pixel-wise spectral loss is sufficient to enforce the global similarity without introducing new modules.

%Spectral loss can be seemed as distance between projections onto the different unitary Fourier basis, which helps the analysis over results. As one point in spectral domain refers to a globally-repeated pattern in spatial domain, spectral loss is a ``half-global'' \footnote{We use the term ``half-global'' as it is not computed over all values.} loss, which can detect some large-area distortion from target image (\textit{e.g.} casted shadow hovering over whole image). 

\subsection{Network Training}\label{subsec:loss}
% As ground truth albedo and shading are available for MPI-Sintel and MIT datasets(\miaojing{keep this unless you want to mention iiw as well }), 

Beside the \textit{spectral loss}, we also adopt representative local MSE loss in the spatial domain to let the predication to be both pixel-wise close and visually similar to the ground truth. Following~\cite{lettry2018darn,fan2018revisiting, narihira2015direct}, we choose the $\ell_2$ loss defined on every pixel value and its gradient:
\begin{align}
\mathcal{L}_p(x,\hat{x}) = \|x- \hat{x}\|_2^2 ,~~~ \mathcal{L}_g(x,\hat{x}) = \|\nabla(x)- \nabla\hat{x}\|_2^2.
\end{align}
Each of the $M$ subbranches in the network is trained with loss $\mathcal{L}_{ss}$ from both spectral and spatial domains:
\begin{align}
\mathcal{L}_{ss}(x,\hat{x}) = \lambda_{1}\mathcal{L}_p +  \lambda_{2}\mathcal{L}_g + \lambda_{3}\mathcal{L}_s. %+ \sum_{\hat{x}_i} \lambda_4^{i}\mathcal{L}_p
\end{align}
We empirically choose $\lambda_1=0.2,\lambda_2=0.35,\lambda_3=10^{-6}$ for all our experiments. \miaojing{$\mathcal{L}_s$ is of larger magnitude than $\mathcal{L}_g$ and $\mathcal{L}_p$ thus with a smaller weight $\lambda_3$.} $\mathcal{L}_{ss}$ is applied to all the $M$ subbranches as well as their final summation in the network, so we have the overall loss $\mathcal{L_T}$ for target albedo/shading:
\begin{align}
\mathcal{L_T} = \sum_{b=1}^{M}\mathcal{L}_{ss}^b(x_b,\hat{x}_b) + \mathcal{L}_{ss}(x,\hat{x}),
\end{align}
where we denote by $x_b$ and $\hat{x}_b$ the ground truth and prediction corresponding to the $b$-th spectral band of the original albedo/shading, respectively. 

Referring to Fig.~\ref{fig:architecture}, 
% we split each spectral residual block chain into two streams after the $\frac{N}{2}$-th block to regress both the albedo ($\mathcal A$) and shading ($\mathcal S$); 
$\mathcal{L_T}$ is computed on both albedo and shading predictions ($\mathcal{L_A}$ and $\mathcal{L_S}$), so we have the final loss
\begin{align}
\mathcal{L} = \mathcal{L_A}  + \mathcal{L_S}  + \mathcal{L_{AS}}
\end{align}
$\mathcal{L_{AS}} = \|\mathcal{A}\cdot\mathcal{S} - \hat{\mathcal A}\cdot\hat{\mathcal S}\|_2^2 $ is added to address the commonly used constraint $\mathcal{I}=\mathcal{A}\cdot\mathcal{S}$ \cite{cheng2018intrinsic}.

%\medskip 
%Notice that FFI-Net can actually be trained with varying loss functions and can thus be treated as a plug-in backbone for main-stream supervised or unsupervised frameworks. In Sec.~\ref{subsec:iiw} we give an example of training a FFI-Net with a single WHDR loss. 

==> WACV2021_ Fourier-Camera Ready/relatedwork.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:relatedwork}
Our main objective is to develop a deep neural network architecture
for intrinsic image decomposition and therefore related works
will focus on the prior deep 
architectures~\cite{narihira2015direct,kim2016unified, fan2018revisiting,lettry2018darn,cheng2018intrinsic,baslamisli2018cnn}. Traditional approaches have
been surveyed in the recent work by Barron and Malik~\cite{barron2015shape}.


%\paragraph{Deep Intrinsic Image Decomposition.}
Nahiriha~\etal~\cite{narihira2015direct} were the first to propose
a deep architecture to estimate albedo and
shading using a pixel-wise MSE loss. Kim~\etal~\cite{kim2016unified} later
added a conditional random field (CRF) after the network to jointly learn albedo, shading and depth.
Lettry~\etal~\cite{lettry2018darn} further proposed to add an adversarial module. To better model the flattening effects in natural reflectance images, Fan \etal \cite{fan2018revisiting} proposed a 1D recursive domain filter and 
separate loss layers customized differently for dense
(\eg MPI-Sintel~\cite{butler2012naturalistic}) and sparse (\eg IIW~\cite{bell2014intrinsic})
datasets; Cheng~\etal~\cite{cheng2018intrinsic} proposed
to use a cross bilateral filtering loss instead of the MSE loss to ensure the smoothness of albedo and shading output. 
Recently, Baslamisli~\textit{et al.}~\cite{baslamisli2018cnn} adopted a physics-based image formation model inspired by traditional approaches.
%Recently, Zhou ~\etal~\cite{zhou2019glosh} propose a global-local spherical harmonics (GLoSH) lighting model to improve the lighting component, and jointly predict reflectance and surface normals.
%Cheng~\etal~\cite{cheng2019non} decoupled reflectance and shading estimation into a convex local shading component based on near-infrared RGB image pair, and a reflectance component based on local and gloabl  reflectance homogeneity. 

The above works assume the Lambertian reflectance model and 
are fully-supervised with ground truth albedo and shading. There are also many works assuming a non-Lambertian model~\cite{shi2017learning}, adopting the weakly-supervised/unsupervised
setting~\cite{janner2017self,li2018learning,ma2018single,liu2020cvpr}, or including more synthetic data for training~\cite{cgintrinsic,zhou2019glosh}. For instance, Shi \etal
\cite{shi2017learning} considered the non-Lambertian model in their algorithm design and train their network with rendered 3D models from ShapeNet~\cite{chang2015shapenet}. 
%Janner \etal \cite{janner2017self} propose a self-supervised learning scheme which transfers learned intrinsic properties to unseen scenes. 
Li \etal \cite{li2018learning} learned intrinsic images from image sequences over time, where the object reflectance remains the same with varying illumination.
%Zhou \etal \cite{zhou2019glosh} apply synthetic data for model pre-training and fine-tune the model with real data in a self-supervised way.
%Ma~\etal~\cite{ma2018single} learn intrinsic representations without supervision by training on multiple images of the same objects. 
Liu \etal \cite{liu2020cvpr} proposed a novel unsupervised intrinsic image decomposition
framework which directly learns the latent feature of reflectance and shading from unsupervised and
uncorrelated data. Zhou \etal \cite{zhou2019glosh} proposed a global-local spherical harmonics lighting model for intrinsic decomposition, where they 
apply synthetic data for model pre-training and fine-tune it with real data in a self-supervised way.
%To enable this, we explore the independence between reflectance and shading, the domain invariant content constraint and the physical constraint.


The FFI-Net is inspired by several recent works while the most important being
~\cite{cheng2018intrinsic, rippel2015spectral}. FFI-Net differs from Cheng \etal~\cite{cheng2018intrinsic} rather substantially in the following ways:
(i) their hierarchical decomposition is done in the spatial domain with fixed-sized Gaussian kernels, while the decomposition in FFI-Net is
made in the spectral domain;
(ii) they use VGG perceptual loss to enforce global similarity between the intrinsic prediction and ground truth while FFI-Net uses the basic
MSE in the spectral domain;
(iii) their network optimization is done in the spatial domain while ours in the spectral domain. With respect to the comparison to~\cite{rippel2015spectral}, FFI-Net adopts the spectral encoding of CNN weights from it but novelly introduces several new elements \ie spectral banding, spectral loss, spectral residual block, for intrinsic image decomposition. 
%Besides, we also enrich several existing elements in~\cite{rippel2015spectral} by offering the complete four conjugate symmetry patterns (Fig.~\ref{fig:conjugate}) as well as encoding the spectral residual blocks (Fig.~\ref{fig:spectralresidualblock}), which can be particularly utilized in the image-to-image translation task. 

==> WACV2021_ Fourier-Camera Ready/tab-iiw.tex <==
\begin{table}
\begin{center}
	\small
\begin{tabular}{llc}
\toprule
Methods & Training set &  WHDR (mean) \\
%& (mean) \\
\midrule
%Baseline (const shading)& -- & 51.37 \\
%Baseline (const reflectance)& -- & 36.54 \\
DI \cite{narihira2015direct} & ST & 37.30 \\
Shen \emph{et al.} \cite{shen2011intrinsic} & -- & 36.90 \\
Retinex (color) \cite{grosse2009ground} & -- & 26.89 \\
Retinex (gray) \cite{grosse2009ground} & -- & 26.84 \\
Garces \emph{et al.} \cite{garces2012intrinsic} & --& 25.46 \\
Zhao \emph{et al.} \cite{zhao2012closed} & -- & 23.20 \\
$L_1$ flattening \cite{bi20151} & -- & 20.94 \\
Bell \emph{et al.} \cite{bell2014intrinsic} & -- & 20.64 \\
Zhou \emph{et al.} \cite{zhou2015learning} & IIW & 19.95 \\
Nestmeyer \emph{et al.} CNN\cite{nestmeyer2017reflectance} & IIW & 19.49 \\
Zoran \emph{et al.} * \cite{zoran2015learning} & IIW & 17.85\\
Nestmeyer \emph{et al.} \cite{nestmeyer2017reflectance} & IIW & 17.69 \\
Bi \emph{et al.} \cite{bi20151}& -- & 17.67 \\
CGI \cite{cgintrinsic} & CGI+IIW & 17.50 \\
CGI \cite{cgintrinsic} & CGI+IIW(A)+SAW & 15.50 \\
Fan \emph{et al.} \cite{fan2018revisiting} & IIW & \textbf{14.45} \\
%Yu \emph{et al.} 2019 %\cite{yu2019inverserendernet} & MegaDepth &21.40 \\
Zhou \etal \cite{zhou2019glosh} & SUNCG + IIW & 15.20 \\
Liu \etal~\cite{liu2020cvpr}  & IIW & 18.69 \\
\midrule
FFI-Net w/ WHDR loss & IIW & {15.81} \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\caption{Results for IIW. Evaluation follows the train-test split in \cite{narihira2015direct}. Note that due to the sparse ground truth available, FFI-Net does not use the spectral banding and loss, but instead the WHDR loss in ~\cite{fan2018revisiting}.
% Minor detail as they are worse than us
%, except for the one marked with * which is evaluated on their own test split and is not directly comparable with other methods.
}
\label{table:iiw}
\vspace{-0.5mm}
\end{table}


==> WACV2021_ Fourier-Camera Ready/tab_mit_A.tex <==
\begin{table}
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\centering
\small
\begin{tabular}{l c cccc}
\toprule
~ & Tr. &
\multicolumn{3}{c}{si-MSE $\times10^{2}$}&\multicolumn{1}{c}{si-LMSE$\times10^{2}$} \cr\cline{3-6}
&data&A&S&avg&Total\cr
\midrule
SIRFS \cite{barron2015shape} & M & 0.64 & 0.98 & 0.81 & 1.25 \cr
\midrule
Zhou \textit{et al.} \cite{zhou2015learning} & M & 2.52 & 2.29 & 2.40 & 3.19 \cr
Shi \textit{et al.} \cite{shi2017learning} & SN+M & 2.16 & 1.35 & 1.75 & 2.71 \cr
DI~\cite{narihira2015direct} & ST+M & 2.07 & 1.24 & 1.65 & 2.39 \cr

%IntriNet(w/o imf)~\cite{baslamisli2018cnn}$^*$ & M & 1.50 & 9.47 & 5.48 & 9.35\cr
%IntriNet(w imf)~\cite{baslamisli2018cnn}$^*$ & M & 1.70 & 7.97 & 4.83 & 7.90\cr
%RetiNet~\cite{baslamisli2018cnn}$^*$ & M & 1.73 & 10.95 & 6.34 & 10.65 \cr

Fan et al.~\cite{fan2018revisiting}& M &  1.34 & 0.89 & 1.11 & 2.03 \cr
LapPyrNet~\cite{cheng2018intrinsic}& I+M &  0.89 & \textbf{0.73} & 0.81 & 1.41  \cr
%\hline
%FFT  ~ & ST & 0.0190 & 0.0185 & 0.0188 & 0.0289 \cr
%FFT  ~ & M & 0.0082 &  0.0077 & 0.0079 & 0.0151 \cr
FFI-Net  ~ & M & \textbf{0.71} &  0.76 & \textbf{0.73} &  \textbf{1.31} \cr % 0.1255 & 0.1129
% ~~w/o $\mathcal L_{\text{spec}}$ & M & 0.82 & 0.77 & 0.79 & 1.52\cr 
%~~M=3 & M & 0.74 & 0.78 & 0.76 & 1.41 \cr
%~~M=1 & M & 0.80 & 0.80 & 0.80 & 1.51 \cr
% ~~cross   & ST & 1.90 & 1.85 & 1.88 &  2.69 \cr 
\bottomrule
\end{tabular}
\caption{
Results for MIT Intrinsic. All methods use the training-test split file released in~\cite{barron2015shape}. 
For si-MSE and si-LMSE, we use the evaluation code from \cite{fan2018revisiting,barron2015shape}. Tr. data lists the datasets used in training: MIT (M), ShapeNet (SN), Sintel (ST) and ImageNet (I). The best CNN-based results are marked in bold. 
%($^\star$ uses prior that is particularly suitable for MIT Intrinsic).
}. 
\label{tab:mit}
\vspace{-2ex}
\end{table}

==> WACV2021_ Fourier-Camera Ready/tab_mit_B.tex <==
\begin{table}
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\centering
\small
\begin{tabular}{l c cccccc}
\hline
~ & Tr. &
\multicolumn{2}{c}{MSE} &\multicolumn{2}{c}{LMSE} &\multicolumn{2}{c}{DSSIM}\cr
\cline{3-8} & data &A&S &A&S &A&S \cr\hline
SIRFS~\cite{barron2015shape} & M & 1.47 & 0.83 & 4.16 & 1.68 & 12.38 &{9.85} \cr
\midrule 
DI~\cite{narihira2015direct} & ST+M & 2.77 & 1.54 & 5.86 & 2.95 & 15.26 &13.28 \cr
%Shi \textit{et al.} \cite{shi2017learning} & SN & 4.68 & 1.94 & 7.52 & 3.18 & 18.25 & 16.67\cr
Shi \textit{et al.} \cite{shi2017learning} & SN+M & 2.78 & 1.26 & 5.03 & 2.40 & 14.65 & 12.00\cr
CGI \cite{cgintrinsic} & CGI & 2.21 & 1.86 & 3.49 & 2.59 & 17.39 & 16.52 \cr
%RetiNet \cite{baslamisli2018cnn} & M & 1.28 & 1.07 & 6.52 & 7.46 & 9.09 & 10.54 \cr  
%IntriNet \cite{baslamisli2018cnn}$^?$ & M & 0.51 & 0.29 & 2.95 & 1.57 & 9.26 & 4.41 \cr
CGI \cite{cgintrinsic} & CGI+M & {1.67} & 1.27 & 3.19 & 2.21 & 12.87 & 13.76 \cr
%Ma \textit{et al.} \cite{ma2018single}$^*$ & -- & 3.13 & 2.07 & 1.16 & 0.95 & -- & -- \cr
Ma \textit{et al.} \cite{ma2018single}$^*$ & M  & 1.68 & {0.93} & {\em 0.74} & {\em 0.52} & -- & -- \cr
Liu \textit{et al.} \cite{liu2020cvpr}
& M & 1.57 & {1.35} & {1.46} & {2.31} & -- & -- \cr
%FFI-Net & M & \textbf{1.11} & 0.94 & {\bf 2.91} & 3.19 & \textbf{10.14} & 13.39 \cr
FFI-Net & M & \textbf{1.11} & \textbf{0.93} & { 2.91} & 3.19 & \textbf{10.14} & \textbf{11.39} \cr
\hline
\end{tabular}
\caption{
More results for MIT Intrinsic under diffferent metrics, MSE, LMSE, and DSSIM (\cite{ma2018single}$^*$ uses a different window size for LMSE). The best CNN-based results are marked in bold. 
}
\label{tab:mit_b}
\vspace{-1ex}
\end{table}

==> WACV2021_ Fourier-Camera Ready/tab_mpi_imagesplit.tex <==
\setlength{\tabcolsep}{1.5pt}
{
\begin{table}[t]
\centering
\resizebox{0.99\linewidth}{!}{
\small
\begin{tabular}{l rrr | rrr | rrr}
\toprule
{Sintel \textit{image split}}&
\multicolumn{3}{c}{si-MSE$\times10^{2}$}&\multicolumn{3}{c}{si-LMSE$\times10^{2}$}&\multicolumn{3}{c}{DSSIM$\times10^{2}$}\\%\cr\cline{2-10}
&A&S&avg&A&S&avg&A&S&avg\\
\midrule
% (??) Baseline: Constant Shading&5.31&4.88&5.10&3.26&2.84&3.05&21.40&20.60&21.00\cr%\hline
% (??) Baseline: Constant Albedo&3.69&3.78&3.74&2.40&3.03&2.72&22.80&18.70&20.75\cr%\hline
Retinex \cite{grosse09intrinsic} ~&6.06&7.27&6.67&3.66&4.19&3.93&22.70&24.00&23.35\cr%\hline
Lee et al. \cite{lee2012estimation}~&4.63&5.07&4.85&2.24&1.92&2.08&19.90&17.70&18.80\cr%\hline
SIRFS~ \cite{barron2015shape}&4.20&4.36&4.28&2.98&2.64&2.81&21.00&20.60&20.80\cr%\hline
Chen et al.~\cite{chen2013simple}&3.07&2.77&2.92&1.85&1.90&1.88&19.60&16.50&18.05\cr%\hline
DI~\cite{narihira2015direct}&1.00&0.92&0.96&0.83&0.85&0.84&20.14&15.05&17.60\cr%\hline
DARN~\cite{lettry2018darn}&1.24&1.28&1.26&0.69&0.70&0.70&12.63&12.13&12.38\cr%\hline
Kim et al.~\cite{kim2016unified}&0.70&0.90&0.70&0.60&0.70&0.70&9.20&10.10&9.70\cr%\hline
Fan et al.~\cite{fan2018revisiting} &0.67& \cellcolor{gray!25}0.60& \cellcolor{gray!25}0.63& \textbf{0.41}& \cellcolor{gray!25}0.42& \textbf{0.41} &10.50&7.83&9.16\cr
LapPyrNet~\cite{cheng2018intrinsic}& \cellcolor{gray!25}0.66 & \cellcolor{gray!25}0.60 & \cellcolor{gray!25}0.63 & \cellcolor{gray!25}0.44 & \cellcolor{gray!25}0.42 & 0.43 & {\bf 6.56} & \cellcolor{gray!25}{6.37} & \textbf{6.47} \cr
Liu \etal \cite{liu2020cvpr} & 1.59 & 1.48 & 1.54 & 0.87 & 0.81 & 0.84 & 17.97 & 14.74 & 16.35 \cr
\midrule
%FFT (use chen split, front)~& 0.62 & 0.64 & 0.63 & 0.43& 0.41 & 0.42 & 8.12 & ~7.13 & 7.62 \cr
%FFT (use chen split, front)~& 0.75 & 0.47 & 0.61 & 0.54 & 0.36 & 0.45 & 9.14 & 6.54 & 7.84 \cr
%FFT (use chen split, reverse)~& 0.67 & 0.50 & 0.58 & 0.48& 0.37 & 0.43 & 8.34 & ~6.43 & 7.40\cr
FFI-Net ~& \textbf{0.64} & \textbf{0.57} & \textbf{0.61} & 0.46 & \textbf{0.39} &  \cellcolor{gray!25}{0.42} & \cellcolor{gray!25}7.73 &  \textbf{6.28} & \cellcolor{gray!25}7.01 \cr
\bottomrule
\end{tabular}}
%}

% $^{*}$ {\small These do no use the same split files \color{red}{with the rest}, but exclude some images or use alternative splittings}
%\cite{fan2018revisiting} exclude several scenes with large masked area; %\cite{cheng2018intrinsic} randomly selected half of images for training and the remainder for testing (from emailing the author).  
\caption{Results for MPI-Sintel (image split). 
%Scores are reported for albedo (A), shading (S) and their average (avg). 
%The best result is marked in bold while the second best in grey.
%Note that Ref.$^1$ excludes some images with large masked area and Ref.$^2$ uses a different split compared to the rest.
}
\vspace{-5mm}
\label{tab:sintel_image_split}.
\end{table}
}

==> WACV2021_ Fourier-Camera Ready/tab_mpi_scenesplit.tex <==
\setlength{\tabcolsep}{1.5pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1} % Default value: 1
{
\begin{table}[t]
\centering
\small
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l rrr | rrr | rrr}
\toprule
{Sintel \textit{scene split}}&
\multicolumn{3}{c}{si-MSE $\times10^{2}$}&\multicolumn{3}{c}{si-LMSE$\times10^{2}$}&\multicolumn{3}{c}{DSSIM$\times10^{2}$}\cr\cline{2-10}
&A&S&avg&A&S&avg&A&S&avg\cr\hline
DI~\cite{narihira2015direct}&2.01&2.24&2.13&1.31&1.48&1.39&20.73&15.94&18.33\cr%\hline
DARN~\cite{lettry2018darn}&1.77&1.84&1.81&0.98&0.95&0.97&14.21&14.05&14.13\cr%\hline
Fan et al.~\cite{fan2018revisiting}&1.81&1.75&1.78&1.22&1.18&1.20&16.74&13.82&15.28\cr
LapPyrNet~\cite{cheng2018intrinsic}& 1.38 & 1.38 & 1.38 & 0.92 & 0.93 & 0.92 & \textbf{8.46} & 9.26 & \cellcolor{gray!25} 8.86 \cr
FFI-Net & \textbf{1.19} &  \textbf{1.16} & \textbf{1.18} & \textbf{0.73} & \textbf{0.73} & \textbf{0.73} &  \cellcolor{gray!25}8.93 & \textbf{8.60} & \textbf{8.77} \cr
\hline
M=5,$R_{\text{spec}}$ & \textbf{1.19} &  \textbf{1.16} & \textbf{1.18} & \textbf{0.73} & \textbf{0.73} & \textbf{0.73} &  \cellcolor{gray!25}8.93 & \textbf{8.60} & \textbf{8.77} \cr
M=3,$R_{\text{spec}}$ & 1.24 &  1.16 & 1.20 & 0.75 & 0.75 & 0.75 &  9.59 & 8.85  & 9.22\\
M=1,$R_{\text{spec}}$ & 1.35 &  1.36 & 1.35 & 0.82 & 0.82 & 0.82 &  10.43 & 10.84 & 10.63\\
M=5,$R_{\text{spat}}$ & 1.50 &  1.50 & 1.50~& 0.91 & 0.92 & 0.91 &  10.25 & 9.78  & 10.01\\
M=3,$R_{\text{spat}}$ & 1.41 &  1.44 & 1.42~& 0.82 & 0.93 & 0.88 &  10.59 & 9.95  & 10.27\\
M=1,$R_{\text{spat}}$ & 1.52 & 1.67 & 1.60&~0.91 & 1.14 & 1.02 & 11.04 & 11.69 & 11.37\\
\hline
%w/  $B_{\text{spat}}$ (M =5, $R_{\text{spec}}$) & {1.29} &  {1.33} & {1.34} & {0.81} & {0.87} & {0.86} & 9.84 & {9.10} & {9.37} \cr
w/o $\mathcal L_{\text{spec}}$ (M =5, $R_{\text{spec}}$) & \textbf{1.19} &  \textbf{1.16} & \textbf{1.18} & \cellcolor{gray!25}0.75 & 0.75 & \cellcolor{gray!25}0.75 &  9.55 &\cellcolor{gray!25}8.70 & 9.13 \cr
only $\mathcal L_{\text{spec}}$ (M =1, $R_{\text{spat}}$) & 1.29 &  1.28 & 1.29 & 0.77 & 0.84 & 0.81 &  10.11 & 9.13 & 9.62 \cr


%FFI-Net \cr
%% ~~(M=1,$L_{\text{spat}}$) & 1.52 & 1.67 & 1.60 & 0.91 & 1.14 & 1.02 & 11.04 & 11.69 & 11.37 \cr
%% ~~(M=1) ~ & 1.35 &  1.36 & 1.35 & 0.82 & 0.82 & 0.82 &  10.43 & 10.84 & 10.63 \cr
%~~(M=5,only $L_{\text{spec}}$) ~ & 1.29 &  1.28 & 1.29 & 0.77 & 0.84 & 0.81 &  10.11 & 9.13 & 9.62 \cr
%% FFI-Net (deconv unsampling) ~ & 1.21 &  \textbf{1.15} & \cellcolor{gray!25}1.18 & 0.76 & 0.73 & \cellcolor{gray!25}0.74 &  9.48 & 8.56 & 9.02 \cr
%~~(M=5,w/o $L_{\text{spec}}$) ~ & \textbf{1.19} &  \textbf{1.16} & \textbf{1.18} & \cellcolor{gray!25}0.75 & 0.75 & \cellcolor{gray!25}0.75 &  9.55 &\cellcolor{gray!25}8.70 & 9.13 \cr
%~~(M=1,$B_{\text{spat}}$) & 1.52 & 1.67 & 1.60&~0.91 & 1.14 & 1.02 & 11.04 & 11.69 & 11.37\\
%~~(M=3,$B_{\text{spat}}$) & 1.41 &  1.44 & 1.42~& 0.82 & 0.93 & 0.88 &  10.59 & 9.95  & 10.27\\
%~~(M=5,$B_{\text{spat}}$) & 1.50 &  1.50 & 1.50~& 0.91 & 0.92 & 0.91 &  10.25 & 9.78  & 10.01\\
%~~(M=1,$B_{\text{spec}}$) & 1.35 &  1.36 & 1.35 & 0.82 & 0.82 & 0.82 &  10.43 & 10.84 & 10.63\\
%~~(M=3,$B_{\text{spec}}$) & 1.24 &  1.16 & 1.20 & 0.75 & 0.75 & 0.75 &  9.59 & 8.85  & 9.22\\
%~~(M=5,$B_{\text{spec}}$)-\textbf{F}  & \textbf{1.19} &  \textbf{1.16} & \textbf{1.18} & \textbf{0.73} & \textbf{0.73} & \textbf{0.73} &  \cellcolor{gray!25}9.03 & \textbf{8.60} & \textbf{8.82} \cr
\bottomrule
\vspace{-3mm}
\end{tabular}
}
\caption{Results for MPI-Sintel (scene split). si-MSE, si-LMSE and DSSIM are reported for albedo (A), shading (S) and their average (avg). We also ablate the key elements of FFI-Net: number of spectral bands $M~\in~\{1,3,5\}$,  spectral ($R_\text{spec}$) vs. spatial ($R_\text{spat}$) residual blocks, 
%spectral banding (by default) vs. spatial banding (w/ $B_\text{spat}$) 
and the spectral loss~$\mathcal L_{\text{spec}}$. FFI-Net is by default with M=5, $R_{\text{spec}}$.
%with $\mathcal L_{\text{spec}}$.
The best results are marked in bold.
%and the second best in grey.
} 
\label{tab:sintel_scene_split}. 
\vspace{-5mm}
\end{table}
}


==> WACV2021_ Fourier-Camera Ready/tables.tex <==
\begin{table*}
\caption{Comparison of color constancy methods. All values are in degrees as defined in angular error. For (a) we retrieve the results of the related works in the following order: 1) the cited paper, 2) Table [1] and Table [2] from Barron \etal \cite{barron2017cvpr} considered to be up-to-date and comprehensive, 3) the color constancy benchmarking website \cite{colorconstancy.com}. We left dash on unreported results. In (a) results of learning-based methods worse than ours are marked in gray. Angular errors with values higher than 10 are reported as $>$10. In the agnostic-camera setting, the proposed algorithm has the best overall performance over both learning-based and statistical methods}
\label{tab:maintable}
\begin{center}
\subfloat[Camera-known setting]{
\label{tab:known}
\begin{threeparttable}
\small
\begin{tabular}{l  rr rrr || rr rrr }

\toprule
    & \multicolumn{5}{c}{SFU Color Checker} & 
    \multicolumn{5}{c}{{NUS 8-camera}} 
    \\%& \multicolumn{4}{c}{SFU Laboratory}\\
    
  & { Mean} & { Median} & Trimean & Best 25\% & Worst 25\% &{ Mean} & { Median} & Trimean & Best 25\% & Worst 25\% \\%& &{\em Mean} & {\em Med} & Trimean \\
\midrule
\multicolumn{5}{c}{{\em Learning-based Methods (camera-known setting)}} \\
Edge-based Gamut ~\cite{gijsenij2010generalized}
 & \cellcolor{gray!25}6.52 & \cellcolor{gray!25}5.04 & \cellcolor{gray!25}5.43 & \cellcolor{gray!25}1.90 & \cellcolor{gray!25}13.58&  \cellcolor{gray!25}4.40  & \cellcolor{gray!25}3.30  & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}0.99 & \cellcolor{gray!25}9.83\\%&& 3.92 &\cellcolor{gray!25}2.28 & \cellcolor{gray!25}2.70 \\ 
 Pixel-based Gamut~\cite{gijsenij2010generalized}
 & \cellcolor{gray!25}4.20 & \cellcolor{gray!25}2.33 & \cellcolor{gray!25}2.91 & \cellcolor{gray!25}0.50 & \cellcolor{gray!25}10.72 &  \cellcolor{gray!25}5.27  & \cellcolor{gray!25}4.26  & \cellcolor{gray!25}4.45 & \cellcolor{gray!25}1.28 & \cellcolor{gray!25}11.16 \\%&& 3.70 & \cellcolor{gray!25}2.27 & 2.3\\
Bayesian \cite{gehler2008bayesian}
%&& 4.82 & 3.46  &  3.88 &&  3.67 & 2.73 & 2.91 && --& --&-- \\
& \cellcolor{gray!25}4.82 & \cellcolor{gray!25}3.46  &  \cellcolor{gray!25}3.88 & \cellcolor{gray!25}1.26 & \cellcolor{gray!25}10.49 & \cellcolor{gray!25}3.50  & \cellcolor{gray!25}2.36 & \cellcolor{gray!25}2.57 & \cellcolor{gray!25}0.78 & \cellcolor{gray!25}8.02\\%&& --& --&-- \\
Natural Image Statistics~\cite{gijsenij2011color}
  & \cellcolor{gray!25}4.19 & \cellcolor{gray!25}3.13 & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}1.00 & \cellcolor{gray!25}9.22& \cellcolor{gray!25}3.45 &  \cellcolor{gray!25}2.88  & \cellcolor{gray!25}2.95 &\cellcolor{gray!25}0.83 & \cellcolor{gray!25}7.18 \\%&& -- & --& --\\
  
 Spatio-spectral (GenPrior) \cite{chakrabarti2012color}
 & \cellcolor{gray!25}3.59  & \cellcolor{gray!25}2.96& \cellcolor{gray!25}3.10 & \cellcolor{gray!25}0.95 & 7.61 &\cellcolor{gray!25}3.06  & \cellcolor{gray!25}2.58  & \cellcolor{gray!25}2.74 & \cellcolor{gray!25}0.87 & 6.17 \\%&& \cellcolor{gray!25}5.63 & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}4.33\\   
 
LSRS  \cite{gao2014eccv}
&  3.31 & \cellcolor{gray!25}2.80  & \cellcolor{gray!25}2.87   & \cellcolor{gray!25}1.14 & 6.39 & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}2.51  & \cellcolor{gray!25}2.70 & \cellcolor{gray!25}0.98 & \cellcolor{gray!25}7.32 \\%&& \cellcolor{gray!25}5.7 & \cellcolor{gray!25}2.4 & \cellcolor{gray!25}4.1\\  
 
Exemplar-based~\cite{joze2014exemplar}
  & 2.89 &  \cellcolor{gray!25}2.27  &\cellcolor{gray!25}2.42  & \cellcolor{gray!25}0.82 & 5.97 & --&-- &--& -- &-- \\
  
Chakrabarti \etal 2015 ~\cite{chakrabarti2015color}
  & 2.56 &  1.67  & 1.89  &\cellcolor{gray!25} 0.52 & 6.07 & --&-- &--& -- &-- \\
  
Cheng \etal 2015 \cite{cheng2015effective}
  & 2.42 &1.65 &1.75 & 0.38 & 5.87 &  2.18  & 1.48  & 1.64 & 0.46 & 5.03 \\%&& 3.26 & 1.75 & 2.12 \\
  
DS-Net (HypNet+SelNet) \cite{shi2016eccv}
  & 1.90  & 1.12 & 1.33 & 0.31 & 4.84 &  2.24  & 1.46 & 1.68 & 0.48 & 6.08 \\%&& -- &-- & -- \\
  
CCC (dist+ext)  \cite{barron2015convolutional} 
  & 1.95 & 1.22 & 1.38 & 0.35 & 4.76 &  2.38 & 1.48 & 1.69 & 0.45 & 5.85 \\%&& -- & --& --\\
FC$^{4}$  (AlexNet) \cite{hu2017cvpr}
& \textbf{1.77} & 1.11 & 1.29 & 0.34 & \textbf{4.29} &  2.12 & 1.53 & 1.67 & 0.48 & 4.78\\%&&  -- & -- & --\\
FFCC  \cite{barron2017cvpr}
  & 1.78 & \textbf{0.96} & \textbf{1.14} & \textbf{0.29} & 4.62 &  \textbf{1.99} & \textbf{1.31} & \textbf{1.43} & \textbf{0.35} & \textbf{4.75}\\%&& --& -- & --\\
\midrule

\textbf{Mean Shifted Grey Pixel}  
& 3.45 &  2.01 & 2.36 & 0.43 & 8.47
& 2.92 & 2.11 & 2.28 & 0.60 & 6.69
\\
\bottomrule
\end{tabular}
\end{threeparttable}
}
   
\subfloat[Camera-agnostic setting]{
\label{tab:agnostic}
\begin{threeparttable}
\small
\begin{tabular}{l  rr rrr || rr rrr  }
\toprule

Training set	&  \multicolumn{5}{c}{{NUS 8-Camera}}  & \multicolumn{5}{c}{{SFU Color Checker}}\\
Testing set 	&  \multicolumn{5}{c}{{SFU Color Checker}}  & \multicolumn{5}{c}{{NUS 8-Camera}}\\
    
				& { Mean} & { Median} & Trimean & Best 25\% & Worst 25\% &{ Mean} & { Median} & Trimean & Best 25\% & Worst 25\% \\%& &{\em Mean} & {\em Med} & Trimean \\

\midrule

\multicolumn{5}{c}{{\em Learning-based Methods (agnostic-camera setting)}} \\
Bayesian \cite{gehler2008bayesian} & $>$10 & $>$10 &$>$10 & $>$10 & $>$10& $>$10 & $>$10 & $>$10& $>$10 & $>$10 \\
Cheng \etal 2015 \cite{Chen-2015-CVPR}  &  5.52 &   4.52 & 4.79& 1.96 & $>$10   & 4.86  & 4.40  &  4.43& 1.72 & 8.87\\ 
RCCNet \cite{yanlin2017iccv} & $>$10 & $>$10 & $>$10 & $>$10 & $>$10& $>$10 & $>$10 & $>$10& $>$10 & $>$10 \\
FFCC \cite{barron2017cvpr}  & 3.91 &  3.15 & 3.34 & 1.22 & \textbf{7.94} & 3.19 &  2.33 & 2.52 & 0.84 & 7.01\\ 
\midrule
\multicolumn{5}{c}{{\em Statistics-based Methods}} \\
White Patch \cite{brainard1986analysis}
& 7.55 &  5.68 & 6.35 & 1.45 & 16.12 & 9.91  & 7.44 &  8.78  & 1.44 & 21.27  \\%&& 9.09 & 6.48 & 7.45\\
Grey World~\cite{buchsbaum1980spatial} & 6.36 &  6.28 & 6.28  & 2.33 & 10.58 & 4.59  & 3.46 &  3.81 & 1.16 & 9.85 \\%&&   	9.78  & 7.00 & 7.60\\
General GW~\cite{barnard2002comparison}
& 4.66  & 3.48 & 3.81 & 1.00 & 10.09 & 3.20 &  2.56 & 2.68 & 0.85 & 6.68\\%&& 5.41 & 3.32 & 3.78\\  
 2st-order grey-Edge ~\cite{van2007edge}
% && 5.13 &4.44& 4.62  && 3.20 & 2.26 & 2.44 && \cellcolor{red!25}5.2 & 2.7& 3.3\\ 
& 5.13 &4.44& 4.62 & 2.11 & 9.26  & 3.36  & 2.70  &2.80 & 0.89 & 7.14\\%&& \cellcolor{red!25}5.19 & 2.74 & 3.25\\ 
1st-order grey-Edge ~\cite{van2007edge}
% && 5.33&4.52& 4.73  && 3.20 & 2.22 & 2.43 && 5.6 & 3.2 & 3.7 \\
 & 5.33&4.52& 4.73 & 1.86 & 10.43 &  3.35  & 2.58 & 2.76 & 0.79 & 7.18\\%&& 5.68 & 3.18 & 3.74 \\
Shades-of-grey \cite{finlayson2004shades}
%&& 4.93 & 4.01 & 4.23  && 3.40  & 2.57  & 2.73 &&  --&-- & -- \\
& 4.93 & 4.01 & 4.23 & 1.14 & 10.20 &  3.67  & 2.94 & 3.03 & 0.99 & 7.75\\%&&  6.4 & 3.7 & 4.6 \\
%Bright Pixels \cite{hrvjoze2012CIC}
% && 3.98 & 2.61& --  && 3.17 & 2.41 & 2.55 && 5.84 &\cellcolor{red!25} 1.90 & --\\ 

Grey Pixel (edge)~\cite{yang2015efficient} & 4.60 &  3.10 & --  & -- & -- & -- & -- & -- & -- & -- \\%&& \cellcolor{yellow!25}5.3 & \cellcolor{yellow!25} 2.3 & -- \\

Cheng et al. 2014 \cite{Cheng14}
& 3.52 & 2.14& 2.47 & 0.50 & 8.74 & 2.93 & 2.33  & 2.42  & 0.78 & \textbf{ 6.13}\\%&& 6.07 &  3.01 &  3.69\\ 
% SVR~\cite{funt2004estimating}\tnote{2}
%  & (p)& -- &  -- & -- & -- & (w)& -- & -- & --  & -- \\

\textbf{Mean Shifted Grey Pixel}  
& \textbf{3.45} &  \textbf{2.01} & \textbf{2.36} & \textbf{0.43} & 8.47
& \textbf{2.92} & \textbf{2.11} & \textbf{2.28} & \textbf{0.60} & 6.69
\\
\bottomrule
\end{tabular}
\end{threeparttable}
}

\end{center}
\end{table*}

==> fig-iiw-supple.tex <==
\begin{figure*}[htb]
  \centering
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    
    

        \vspace{-1mm}
        \\  
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881-albedo.png}& 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/23881-shading.png}
  
          \vspace{-1mm}
        \\  
        %% 3rd row
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122-albedo.png}& 
                \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/106122-shading.png}
                
%           \vspace{-1mm}
%         \\  
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_img.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_bell_A.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_bell_S.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_zhou_A.jpg} & 
% 		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_zhou_S.jpg} &         
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_cg_A.jpg}  & 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735_cg_S.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735-albedo.png}& 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/34735-shading.png}
        
        
                  \vspace{-1mm}
        \\  
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54-albedo.png}& 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/54-shading.png}

                  \vspace{-1mm}
        \\  
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_img.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_bell_A.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_bell_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_zhou_A.jpg} & 
		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_zhou_S.jpg} &         
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_cg_A.jpg}  & 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155_cg_S.jpg} &
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155-albedo.png}& 
        \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw_supple/6155-shading.png}


%         \vspace{-1mm}
%         \\  
%         %% 3rd row
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/img/118514.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/bell/118514-r.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/bell/118514-s.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/118514-r.jpg} & 
% 		\includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/zhou/118514-s.jpg} &         
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/118514-r.jpg}  & 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/cg/118514-s.jpg} &
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/118514-albedo.png}& 
%         \includegraphics[width=0.11\textwidth,height=0.07\textwidth]{comp_iiw/ffi/118514-shading.png}
        
    
         \vspace{-1mm}
        \\                       
        {\scriptsize Image} & {\scriptsize Bell~\cite{bell2014intrinsic} ($A$)}  & {\scriptsize Bell~\cite{bell2014intrinsic}($S$)} & {\scriptsize Zhou~\cite{zhou2015learning} ($A$)}  & {\scriptsize Zhou \cite{zhou2015learning} ($S$)}  & {\scriptsize CGI \cite{cgintrinsic} ($A$)} & {\scriptsize CGI \cite{cgintrinsic} ($S$)}   &  {\scriptsize FFI-Net ($A$)} & {\scriptsize FFI-Net ($S$)}
    \end{tabular}  
  \caption{ Qualitative comparisons of (A)lebdo and (S)hading on IIW.
    % Our predictions show significant improvements compared to
    % state-of-the-art algorithms (bell~\etal ~\cite{bell2014intrinsic}
    % and zhou~\etal~\cite{zhou2015learning}). 
    % In particular, our
    % predicted shading channels include significantly less surface
    % texture in several challenging
    % settings.
    } \label{fig:iiw} 
\end{figure*}

==> fig-iiw-withsota.tex <==
% \setlength{\tabcolsep}{0.1pt}
% \renewcommand{\arraystretch}{1}
\begin{figure*}
\centering
%\begin{tabular}{ccccccc}
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155.png}& 
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_am_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_am_our.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155-albedo.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_shading_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155_shading_our.png} &
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/6155-shading.png} \\
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940.png}& 
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_am_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_am.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940-albedo.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_shading_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940_shading.png} &
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/7940-shading.png} \\
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54.png}& 
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_am_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_am.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54-albedo.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_shading_li.png}&
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54_shading.png} &
\includegraphics[width=2.4cm,height=1.8cm]{IIW4/54-shading.png} \\
Images & Li \cite{BigTimeLi18} (A) & \cite{yu2019inverserendernet} (A) & FFI-Net (A) & Li \cite{BigTimeLi18} (S) &  \cite{yu2019inverserendernet} (S) & FFI-Net (S)\\
\end{tabular}
    \vspace{-0.2cm}
    \caption{Qualitative comparison with latest SoTAs for IIW. Second column to forth column are reflectance predictions from Li~\cite{BigTimeLi18}, InverseRenderNet~\cite{yu2019inverserendernet} and ours.}
     \label{fig:iiw-with-sota}
\end{figure*}

==> fig-mit-supple.tex <==
%\setlength{\tabcolsep}{0.1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[htp]
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c c ccccc}
\vspace{-0.5mm}
\!\!\includegraphics[width=1.4cm]{comp_MIT/turtle_input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo_di.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo_fan.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_albedo.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_label_albedo.jpg}\cr
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading_di.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading_fan.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/turtle_predict_shading.jpg}\\

\vspace{-0.5mm}

\!\!\includegraphics[width=1.4cm]{comp_MIT/deer_input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo_di.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo_fan.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_albedo.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_label_albedo.jpg}
\\
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_shading_shi.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_shading_di.jpg}
&\includegraphics[width=1.4cm,,height=1.215cm]{comp_MIT/deer_predict_shading_fan.jpg}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/deer_predict_shading.jpg}
&\includegraphics[width=1.4cm]{comp_MIT/deer_predict_shading.jpg}\\

%\vspace{-0.75mm}
%
%\includegraphics[width=1.4cm]{pear-1-input.jpg}
%
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo-Shijian.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo-DI.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-albedo.jpg}
%&\includegraphics[width=1.4cm]{pear-1-labelA.jpg}
%
%&\includegraphics[width=1.4cm]{pear-1-predict-shading-Shijian.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-shading-DI.jpg}
%&\includegraphics[width=1.4cm]{pear-1-predict-shading.jpg}
%&\includegraphics[width=1.4cm]{pear-1-labelS.jpg}\\

%\vspace{-0.75mm}
%
%\includegraphics[width=1.4cm]{turtle-1-input.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo-Shijian.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo-DI.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-albedo.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-labelA.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading-Shijian.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading-DI.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-predict-shading.jpg}
%&\includegraphics[width=1.4cm]{turtle-1-labelS.jpg}\\

\vspace{-0.5mm}

\small{Input} & & \small{Shi \emph{et al.} \cite{shi2017learning}} & \small{DI \cite{narihira2015direct}} & \small{Fan \textit{et al.} \cite{fan2018revisiting}} & \small{FFI-Net} & \small{Ground Truth}\\

% \vspace{-0.6mm}

% &\multicolumn{4}{ c }{\small{Albedo}} & \multicolumn{4}{ c }{\small{Shading}}\\
\end{tabular}}

\end{center}
\vspace{-2mm}
\caption{Sample  (A)lbedo and (S)hading on MIT Intrinsic. 
%Only trained on MIT itself, our method can produce visually-pleasing output, similiar to Fan \textit{et al.} \cite{fan2018revisiting}
}
\label{figure:mit-supple}
\vspace{-0mm}
\end{figure}


==> fig-mit2.tex <==
%\setlength{\tabcolsep}{0.1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[htp]
\begin{center}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c c ccccc}
\vspace{-0.5mm}
\!\!\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_no_imf_turtle_albedo.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_yes_imf_turtle_albedo.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/retinet_turtle_albedo.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_predict_albedo.jpg}
&\includegraphics[width=1.4cm,,height=1cm]{comp_MIT/turtle_label_albedo.jpg}
\cr
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_no_imf_turtle_shading.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/intrinet_yes_imf_turtle_shading.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT2/retinet_turtle_shading.png}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_predict_shading.jpg}
&\includegraphics[width=1.4cm,height=1.cm]{comp_MIT/turtle_label_shading.jpg}
\\

\vspace{-0.5mm}

\!\!\includegraphics[width=1.4cm]{comp_MIT/paper2-1-input.jpg}
& \raisebox{3mm}{\rotatebox{0}{(A)}}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_no_imf_paper2_albedo.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_yes_imf_paper2_albedo.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/retinet_paper2_albedo.png}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/paper2-1-predict-albedo.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT/paper2-1-labelA.jpg}\\
& \raisebox{3mm}{\rotatebox{0}{(S)}}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_no_imf_paper2_shading.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/intrinet_yes_imf_paper2_shading.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT2/retinet_paper2_shading.png}
&\includegraphics[width=1.4cm, height=1.215cm]{comp_MIT/paper2-1-predict-shading.png}
&\includegraphics[width=1.4cm,height=1.215cm]{comp_MIT/paper2-1-labelS.jpg}\\

\vspace{-0.5mm}

\small{Input} & & IntriNet  & IntriNet  & Retinet & \small{FFI-Net} & \small{Ground Truth}\\
 & & w/o imf\cite{baslamisli2018cnn} &  w/ imf\cite{baslamisli2018cnn} & \cite{baslamisli2018cnn} &  & \\

% \vspace{-0.6mm}

% &\multicolumn{4}{ c }{\small{Albedo}} & \multicolumn{4}{ c }{\small{Shading}}\\
\end{tabular}}

\end{center}
\vspace{-2mm}
\caption{Sample  (A)lbedo and (S)hading on MIT Intrinsic. Comparison with different versions in~\cite{baslamisli2018cnn}. Results of~\cite{baslamisli2018cnn} are downloaded from their project webpage.
%Only trained on MIT itself, our method can produce visually-pleasing output, similiar to Fan \textit{et al.} \cite{fan2018revisiting}
}
\vspace{-3mm}
\label{figure:mit2}
\end{figure}


==> fig-mpi-imagesplit-supple.tex <==
%\setlength{\tabcolsep}{1pt}
%\renewcommand{\arraystretch}{1}
\begin{figure}[t]
\begin{center}

%\begin{tabular}{cccc}
%
%%\vspace{-0.75mm}
%%\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%%&\multicolumn{2}{ c }{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}} \\
%%
%%\vspace{-0.75mm}
%%\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}\\
%%
%%\vspace{-0.75mm}
%%\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}\\
%%
%%\vspace{-0.75mm}
%%{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}} &
%%\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg} & \includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg} & \includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}\\
%%&\scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} & \scriptsize{\textbf{Albedo}} & \scriptsize{\textbf{Shading}} \\
%
%\vspace{-0.75mm}
%&\raisebox{.9\height}{\rotatebox{90}{\scriptsize{\textbf{Input}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-input.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-input.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.5\height}{\rotatebox{90}{\scriptsize{\textbf{Albedo}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-albedo.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-albedo.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-albedo.jpg}}}\\
%
%\cmidrule{3-4}
%\multirow{3}{*}{\raisebox{-1.3\height}{\rotatebox{90}{\scriptsize{\textbf{Shading}}}}}
%\vspace{-0.75mm}
%&\raisebox{.6\height}{\rotatebox{90}{\scriptsize{\textbf{MSCR}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading-DI.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading-DI.jpg}}}\\
%
%\vspace{-0.75mm}
%&\raisebox{1\height}{\rotatebox{90}{\scriptsize{\textbf{Ours}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-predict-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-predict-shading.jpg}}}\\
%
%\vspace{-0.75mm}
%&{\rotatebox{90}{\scriptsize{\textbf{Ground Truth}}}}
%&{{\includegraphics[width=3.5cm]{alley_2_frame_0047-label-shading.jpg}}}
%&{{\includegraphics[width=3.5cm]{bamboo_2_frame_0044-label-shading.jpg}}}\\
%
%\end{tabular}

\begin{tabular}{ccc}

\vspace{-0.75mm}
\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}
&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-input.jpg}}
\\
& (A) & (S) \\
% \vspace{-0.75mm}
% \raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Lee~\cite{lee2012estimation}}}}}
% &{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-lee.jpg}}}
% &{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-lee.jpg}}}
% \\

\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Barron~\cite{barron2015shape}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-barron.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-barron.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{0.5\height}{\rotatebox{90}{\scriptsize{{Chen~\cite{chen2013simple}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-chen.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-chen.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-di.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-di.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-fan.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-fan.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Lap\cite{cheng2018intrinsic}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-lap.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-lap.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-albedo-fft.png}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-predict-shading-fft.png}}}
\\

\vspace{-0.75mm}
{\rotatebox{90}{\scriptsize{{Ground Truth}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-label-albedo-mark.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-imagesplit/2-label-shading-mark.jpg}}}
\\
\vspace{-5mm}

\end{tabular}


\end{center}
\vspace{-2.5mm}
\caption{More Examples of (A)lbedo and (S)hading predictions on MPI-Sintel (image split). %FFI-Net performs well in difficult parts, \eg hair bunchesa and  cast shadows.
}
\label{figure:mpi_imagesplit_supple}
\vspace{-3mm}
\end{figure}

%Compared to state-of-the-art method MSCR \cite{DI2015}, we show much sharper effects and better performance.


==> fig-mpi-scensplit-supple.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1}
\begin{figure}
\begin{center}
\vspace{-3mm}
\begin{tabular}{ccc}

%\vspace{-0.75mm}
%\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-input.jpg}}\\& (A) & (S) \\
%\vspace{-0.75mm}
%\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-albedo-MSCR.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-shading-MSCR.jpg}}}\\

%\vspace{-0.75mm} \raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-albedo-fan.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-shading-fan.jpg}}}\\

%\vspace{-0.75mm}
%\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-albedo.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-predict-shading.jpg}}}\\

%\vspace{-0.75mm}
%{\rotatebox{90}{\scriptsize{{Ground Truth}}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-label-albedo.jpg}}}&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/sleeping_2_frame_0014-label-shading.jpg}}}\vspace{5mm}\\

\raisebox{.9\height}{\rotatebox{90}{\scriptsize{{Input}}}}
&\multicolumn{2}{c}{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-input.jpg}}
\\
& (A) & (S) \\
\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{DI~\cite{narihira2015direct}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-albedo-MSCR.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-shading-MSCR.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{Fan \cite{fan2018revisiting}}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-albedo-fan.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-shading-fan.jpg}}}
\\

\vspace{-0.75mm}
\raisebox{1\height}{\rotatebox{90}{\scriptsize{{~~~~FFI}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-albedo.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-predict-shading.jpg}}}
\\

\vspace{-0.75mm}
{\rotatebox{90}{\scriptsize{{Ground Truth}}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-label-albedo-mark.jpg}}}
&{{\includegraphics[width=3.6cm]{comp-mpi-scenesplit/market_6_frame_0012-label-shading-mark.jpg}}}
\\


\vspace{-5mm}

\end{tabular}

\end{center}
\vspace{-2.5mm}
\caption{Examples on the MPI-Sintel dataset (scene split). }
\label{figure:mpi_scenesplit_supple}
%\vspace{-3mm}
\end{figure}

%Compared to state-of-the-art method MSCR \cite{DI2015}, we show much sharper effects and better performance.


==> tables.tex <==
\begin{table*}
\caption{Comparison of color constancy methods. All values are in degrees as defined in angular error. For (a) we retrieve the results of the related works in the following order: 1) the cited paper, 2) Table [1] and Table [2] from Barron \etal \cite{barron2017cvpr} considered to be up-to-date and comprehensive, 3) the color constancy benchmarking website \cite{colorconstancy.com}. We left dash on unreported results. In (a) results of learning-based methods worse than ours are marked in gray. Angular errors with values higher than 10 are reported as $>$10. In the agnostic-camera setting, the proposed algorithm has the best overall performance over both learning-based and statistical methods}
\label{tab:maintable}
\begin{center}
\subfloat[Camera-known setting]{
\label{tab:known}
\begin{threeparttable}
\small
\begin{tabular}{l  rr rrr || rr rrr }

\toprule
    & \multicolumn{5}{c}{SFU Color Checker} & 
    \multicolumn{5}{c}{{NUS 8-camera}} 
    \\%& \multicolumn{4}{c}{SFU Laboratory}\\
    
  & { Mean} & { Median} & Trimean & Best 25\% & Worst 25\% &{ Mean} & { Median} & Trimean & Best 25\% & Worst 25\% \\%& &{\em Mean} & {\em Med} & Trimean \\
\midrule
\multicolumn{5}{c}{{\em Learning-based Methods (camera-known setting)}} \\
Edge-based Gamut ~\cite{gijsenij2010generalized}
 & \cellcolor{gray!25}6.52 & \cellcolor{gray!25}5.04 & \cellcolor{gray!25}5.43 & \cellcolor{gray!25}1.90 & \cellcolor{gray!25}13.58&  \cellcolor{gray!25}4.40  & \cellcolor{gray!25}3.30  & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}0.99 & \cellcolor{gray!25}9.83\\%&& 3.92 &\cellcolor{gray!25}2.28 & \cellcolor{gray!25}2.70 \\ 
 Pixel-based Gamut~\cite{gijsenij2010generalized}
 & \cellcolor{gray!25}4.20 & \cellcolor{gray!25}2.33 & \cellcolor{gray!25}2.91 & \cellcolor{gray!25}0.50 & \cellcolor{gray!25}10.72 &  \cellcolor{gray!25}5.27  & \cellcolor{gray!25}4.26  & \cellcolor{gray!25}4.45 & \cellcolor{gray!25}1.28 & \cellcolor{gray!25}11.16 \\%&& 3.70 & \cellcolor{gray!25}2.27 & 2.3\\
Bayesian \cite{gehler2008bayesian}
%&& 4.82 & 3.46  &  3.88 &&  3.67 & 2.73 & 2.91 && --& --&-- \\
& \cellcolor{gray!25}4.82 & \cellcolor{gray!25}3.46  &  \cellcolor{gray!25}3.88 & \cellcolor{gray!25}1.26 & \cellcolor{gray!25}10.49 & \cellcolor{gray!25}3.50  & \cellcolor{gray!25}2.36 & \cellcolor{gray!25}2.57 & \cellcolor{gray!25}0.78 & \cellcolor{gray!25}8.02\\%&& --& --&-- \\
Natural Image Statistics~\cite{gijsenij2011color}
  & \cellcolor{gray!25}4.19 & \cellcolor{gray!25}3.13 & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}1.00 & \cellcolor{gray!25}9.22& \cellcolor{gray!25}3.45 &  \cellcolor{gray!25}2.88  & \cellcolor{gray!25}2.95 &\cellcolor{gray!25}0.83 & \cellcolor{gray!25}7.18 \\%&& -- & --& --\\
  
 Spatio-spectral (GenPrior) \cite{chakrabarti2012color}
 & \cellcolor{gray!25}3.59  & \cellcolor{gray!25}2.96& \cellcolor{gray!25}3.10 & \cellcolor{gray!25}0.95 & 7.61 &\cellcolor{gray!25}3.06  & \cellcolor{gray!25}2.58  & \cellcolor{gray!25}2.74 & \cellcolor{gray!25}0.87 & 6.17 \\%&& \cellcolor{gray!25}5.63 & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}4.33\\   
 
LSRS  \cite{gao2014eccv}
&  3.31 & \cellcolor{gray!25}2.80  & \cellcolor{gray!25}2.87   & \cellcolor{gray!25}1.14 & 6.39 & \cellcolor{gray!25}3.45 & \cellcolor{gray!25}2.51  & \cellcolor{gray!25}2.70 & \cellcolor{gray!25}0.98 & \cellcolor{gray!25}7.32 \\%&& \cellcolor{gray!25}5.7 & \cellcolor{gray!25}2.4 & \cellcolor{gray!25}4.1\\  
 
Exemplar-based~\cite{joze2014exemplar}
  & 2.89 &  \cellcolor{gray!25}2.27  &\cellcolor{gray!25}2.42  & \cellcolor{gray!25}0.82 & 5.97 & --&-- &--& -- &-- \\
  
Chakrabarti \etal 2015 ~\cite{chakrabarti2015color}
  & 2.56 &  1.67  & 1.89  &\cellcolor{gray!25} 0.52 & 6.07 & --&-- &--& -- &-- \\
  
Cheng \etal 2015 \cite{cheng2015effective}
  & 2.42 &1.65 &1.75 & 0.38 & 5.87 &  2.18  & 1.48  & 1.64 & 0.46 & 5.03 \\%&& 3.26 & 1.75 & 2.12 \\
  
DS-Net (HypNet+SelNet) \cite{shi2016eccv}
  & 1.90  & 1.12 & 1.33 & 0.31 & 4.84 &  2.24  & 1.46 & 1.68 & 0.48 & 6.08 \\%&& -- &-- & -- \\
  
CCC (dist+ext)  \cite{barron2015convolutional} 
  & 1.95 & 1.22 & 1.38 & 0.35 & 4.76 &  2.38 & 1.48 & 1.69 & 0.45 & 5.85 \\%&& -- & --& --\\
FC$^{4}$  (AlexNet) \cite{hu2017cvpr}
& \textbf{1.77} & 1.11 & 1.29 & 0.34 & \textbf{4.29} &  2.12 & 1.53 & 1.67 & 0.48 & 4.78\\%&&  -- & -- & --\\
FFCC  \cite{barron2017cvpr}
  & 1.78 & \textbf{0.96} & \textbf{1.14} & \textbf{0.29} & 4.62 &  \textbf{1.99} & \textbf{1.31} & \textbf{1.43} & \textbf{0.35} & \textbf{4.75}\\%&& --& -- & --\\
\midrule

\textbf{Mean Shifted Grey Pixel}  
& 3.45 &  2.01 & 2.36 & 0.43 & 8.47
& 2.92 & 2.11 & 2.28 & 0.60 & 6.69
\\
\bottomrule
\end{tabular}
\end{threeparttable}
}
   
\subfloat[Camera-agnostic setting]{
\label{tab:agnostic}
\begin{threeparttable}
\small
\begin{tabular}{l  rr rrr || rr rrr  }
\toprule

Training set	&  \multicolumn{5}{c}{{NUS 8-Camera}}  & \multicolumn{5}{c}{{SFU Color Checker}}\\
Testing set 	&  \multicolumn{5}{c}{{SFU Color Checker}}  & \multicolumn{5}{c}{{NUS 8-Camera}}\\
    
				& { Mean} & { Median} & Trimean & Best 25\% & Worst 25\% &{ Mean} & { Median} & Trimean & Best 25\% & Worst 25\% \\%& &{\em Mean} & {\em Med} & Trimean \\

\midrule

\multicolumn{5}{c}{{\em Learning-based Methods (agnostic-camera setting)}} \\
Bayesian \cite{gehler2008bayesian} & $>$10 & $>$10 &$>$10 & $>$10 & $>$10& $>$10 & $>$10 & $>$10& $>$10 & $>$10 \\
Cheng \etal 2015 \cite{Chen-2015-CVPR}  &  5.52 &   4.52 & 4.79& 1.96 & $>$10   & 4.86  & 4.40  &  4.43& 1.72 & 8.87\\ 
RCCNet \cite{yanlin2017iccv} & $>$10 & $>$10 & $>$10 & $>$10 & $>$10& $>$10 & $>$10 & $>$10& $>$10 & $>$10 \\
FFCC \cite{barron2017cvpr}  & 3.91 &  3.15 & 3.34 & 1.22 & \textbf{7.94} & 3.19 &  2.33 & 2.52 & 0.84 & 7.01\\ 
\midrule
\multicolumn{5}{c}{{\em Statistics-based Methods}} \\
White Patch \cite{brainard1986analysis}
& 7.55 &  5.68 & 6.35 & 1.45 & 16.12 & 9.91  & 7.44 &  8.78  & 1.44 & 21.27  \\%&& 9.09 & 6.48 & 7.45\\
Grey World~\cite{buchsbaum1980spatial} & 6.36 &  6.28 & 6.28  & 2.33 & 10.58 & 4.59  & 3.46 &  3.81 & 1.16 & 9.85 \\%&&   	9.78  & 7.00 & 7.60\\
General GW~\cite{barnard2002comparison}
& 4.66  & 3.48 & 3.81 & 1.00 & 10.09 & 3.20 &  2.56 & 2.68 & 0.85 & 6.68\\%&& 5.41 & 3.32 & 3.78\\  
 2st-order grey-Edge ~\cite{van2007edge}
% && 5.13 &4.44& 4.62  && 3.20 & 2.26 & 2.44 && \cellcolor{red!25}5.2 & 2.7& 3.3\\ 
& 5.13 &4.44& 4.62 & 2.11 & 9.26  & 3.36  & 2.70  &2.80 & 0.89 & 7.14\\%&& \cellcolor{red!25}5.19 & 2.74 & 3.25\\ 
1st-order grey-Edge ~\cite{van2007edge}
% && 5.33&4.52& 4.73  && 3.20 & 2.22 & 2.43 && 5.6 & 3.2 & 3.7 \\
 & 5.33&4.52& 4.73 & 1.86 & 10.43 &  3.35  & 2.58 & 2.76 & 0.79 & 7.18\\%&& 5.68 & 3.18 & 3.74 \\
Shades-of-grey \cite{finlayson2004shades}
%&& 4.93 & 4.01 & 4.23  && 3.40  & 2.57  & 2.73 &&  --&-- & -- \\
& 4.93 & 4.01 & 4.23 & 1.14 & 10.20 &  3.67  & 2.94 & 3.03 & 0.99 & 7.75\\%&&  6.4 & 3.7 & 4.6 \\
%Bright Pixels \cite{hrvjoze2012CIC}
% && 3.98 & 2.61& --  && 3.17 & 2.41 & 2.55 && 5.84 &\cellcolor{red!25} 1.90 & --\\ 

Grey Pixel (edge)~\cite{yang2015efficient} & 4.60 &  3.10 & --  & -- & -- & -- & -- & -- & -- & -- \\%&& \cellcolor{yellow!25}5.3 & \cellcolor{yellow!25} 2.3 & -- \\

Cheng et al. 2014 \cite{Cheng14}
& 3.52 & 2.14& 2.47 & 0.50 & 8.74 & 2.93 & 2.33  & 2.42  & 0.78 & \textbf{ 6.13}\\%&& 6.07 &  3.01 &  3.69\\ 
% SVR~\cite{funt2004estimating}\tnote{2}
%  & (p)& -- &  -- & -- & -- & (w)& -- & -- & --  & -- \\

\textbf{Mean Shifted Grey Pixel}  
& \textbf{3.45} &  \textbf{2.01} & \textbf{2.36} & \textbf{0.43} & 8.47
& \textbf{2.92} & \textbf{2.11} & \textbf{2.28} & \textbf{0.60} & 6.69
\\
\bottomrule
\end{tabular}
\end{threeparttable}
}

\end{center}
\end{table*}
